A latent process model for monitoring progress towards hard-to-measure targets, with applications to mental health and online educational assessments

The recent shift to remote learning and work has aggravated long-standing problems, such as the problem of monitoring the mental health of individuals and the progress of students towards learning targets. We introduce a novel latent process model with a view to monitoring the progress of individuals towards a hard-to-measure target of interest, measured by a set of variables. The latent process model is based on the idea of embedding both individuals and variables measuring progress towards the target of interest in a shared metric space, interpreted as an interaction map that captures interactions between individuals and variables. The fact that individuals are embedded in the same metric space as the target helps assess the progress of individuals towards the target. We demonstrate, with the help of simulations and applications, that the latent process model enables a novel look at mental health and online educational assessments in disadvantaged subpopulations.

==> andersen.tex <==
A classic approach to measuring progress of students in educational assessments is based on \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model.

\citeauthor{andersen:85}'s (\citeyear{andersen:85}) model assumes that binary responses $Y_{i,j,t} \in \{0, 1\}$ are independent $\mbox{Bernoulli}(\mu_{i,j,t})$ random variables with log odds
\beno
\eta_{i,j,t}
&=& \log \dfrac{\mu_{i,j,t}}{1-\mu_{i,j,t}}
&\coloneqq& \alpha_{i,t} + \beta_j.
\ee
To compare \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model with the latent process model,
consider binary responses $Y_{i,j,t} \in \{0, 1\}$ by students $i$ to items $j$ at $T = 2$ time points $t \in \{1, 2\}$ along with the following reparameterization of \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model:
\beno
\alpha_{i,1} \;\;\coloneqq\;\; -\gamma\, d(\bm{a}_{i,1},\, \mT)\s
\\
\alpha_{i,2}
\;\;\coloneqq\;\; -\gamma\, d(\bm{a}_{i,2},\, \mT)
\;\;=\;\; -\gamma\, (1 - \lambda_{i,2})\, d(\bm{a}_{i,1},\, \mT)
\;\;=\;\; (1 - \lambda_{i,2})\; \alpha_{i,1},
\ee
where $\gamma \in [0, +\infty)$,
$d(\bm{a}_{i,t}, \mT) \coloneqq |\!|\bm{a}_{i,t} - \mT|\!|_2$ ($t \in \{1, 2\}$),
and $d(\bm{a}_{i,2},\, \mT) = (1 - \lambda_{i,2})\; \alpha_{i,1}$ by Equation \eqref{d.reduction} in Section \ref{special.cases}.

Then,
under \citeauthor{andersen:85}'s (\citeyear{andersen:85}) reparameterized model,
the rate of progress $\lambda_{i,2}$ of student $i$ between time $1$ and $2$ is a function of the distances $d(\bm{a}_{i,1},\, \mT)$ and $d(\bm{a}_{i,2},\, \mT)$:
\beno
\lambda_{i,2}
&=& 1 - \dfrac{\alpha_{i,2}}{\alpha_{i,1}}
&=& 1 - \dfrac{d(\bm{a}_{i,2},\, \mT)}{d(\bm{a}_{i,1},\, \mT)},
\ee
provided that $d(\bm{a}_{i,1},\, \mT) > 0$.
As a result,
\bi
\item the abilities $\alpha_{i,1}$ and $\alpha_{i,2}$ of student $i$ at time $1$ and $2$ can be interpreted in terms of distances $d(\bm{a}_{i,1},\, \mT)$ and $d(\bm{a}_{i,2},\, \mT)$ between student $i$ and learning target $\mT$ in an underlying metric space $(\mathbb{M},\, d)$,\vspace{.1cm}
\item $1 - \alpha_{i,2}\, / \alpha_{i,1}$ can be interpreted as the rate of progress of student $i$ towards learning target $\mT$.
\ei

That being said,
\citeauthor{andersen:85}'s (\citeyear{andersen:85}) model has two limitations:\vspace{.1cm}
\begin{enumerate}
\item {\bf \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model does not capture interactions:} 
\citeauthor{andersen:85}'s (\citeyear{andersen:85}) model assumes that the log odds
\beno
\eta_{i,j,t}
&=& \log \dfrac{\mu_{i,j,t}}{1-\mu_{i,j,t}}
&\coloneqq& \alpha_{i,t} + \beta_j
\ee
is additive in the ability $\alpha_{i,t}$ of student $i$ at time $t$ and the easiness $\beta_j$ of item $j$ and therefore does not capture interactions between students $i$ and items $j$ arising from unobserved variables,
such as cultural background, upbringing, and mentoring.
As a result,
the underlying metric space $(\mathbb{M},\, d)$ of \citeauthor{andersen:85}'s (\citeyear{andersen:85}) reparameterized model cannot be interpreted as an interaction map,
but should be interpreted as an ability map:
In fact,
the distances $d(\bm{a}_{i,1},\, \mT) = -\alpha_{i,1}\, /\, \gamma \propto -\alpha_{i,1} \in [0,\, +\infty)$ and $d(\bm{a}_{i,2},\, \mT) = -\alpha_{i,2}\, /\, \gamma \propto -\alpha_{i,2} \in [0,\, +\infty)$ of individual $i$ to target $\mT$ at time $1$ and $2$ are proportional to the abilities $\alpha_{i,1}$ and $\alpha_{i,2}$.
By contrast,
the latent process model assumes that the log odds is
\beno
\eta_{i,j,t}
&=& \log \dfrac{\mu_{i,j,t}}{1-\mu_{i,j,t}}
&\coloneqq&
\begin{cases}
\alpha_i + \beta_j - \gamma\; d(\bm{a}_{i,1}, \bm{b}_j)
& \mbox{if } t = 1\s
\\
\alpha_i + \beta_j - \gamma\; d(\bm{a}_{i,2}, \mT)
& \mbox{if } t = 2.
\end{cases}
\ee
As a consequence,
the latent process model can capture interactions between individuals (e.g., students) and variables (e.g., items):
e.g.,
in educational assessments,
a large distance between student $i$ and item $j$ indicates that the probability of a correct response of student $i$ to item $j$ is lower than would be expected based on the potential (ability) $\alpha_i$ of student $i$ and the easiness $\beta_j$ of item $j$.
Thus,
the underlying metric space $(\mathbb{M},\, d)$ of the latent process model should be interpreted as an interaction map rather than an ability map.
A simulation study in Section \ref{sec:interaction} confirms that the latent process model can capture interactions between students and items,
whereas \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model does not capture interactions.\vspace{.1cm}
\item {\bf \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model provides one-dimensional ability maps:}
The fact that the metric space $(\mathbb{M},\, d)$ underlying \citeauthor{andersen:85}'s (\citeyear{andersen:85}) reparameterized model represents an ability map gives rise to an additional limitation of \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model:
If,
e.g.,
$\mathbb{M} \coloneqq \mR^q$ ($q \geq 1$) and $d(\bm{a}_{i,t}, \mT) \coloneqq |\!|\bm{a}_{i,t} - \mT|\!|_2$,
then $q=1$ dimension is sufficient for representing the distances $d(\bm{a}_{i,t}, \mT)$ between individuals $i$ at time $t$ and learning target $\mT$ in $(\mathbb{M},\, d)$.
A Euclidean space $\mR^q$ of dimension $q \geq 2$ would provide a less parsimonious representation than $q = 1$ and therefore $q = 1$ is preferable to $q \geq 2$ according to Occam's razor \citep{JeBe92}.
By contrast,
the metric space $(\mathbb{M},\, d)$ underlying the latent process model represents an interaction map rather than an ability map.
To capture interactions between students and items,
a Euclidean space $\mR^q$ of dimension $q \geq 2$ may be required.
% The applications in Sections \ref{sec:depression} and \ref{sec:math} demonstrate that.
\hide{
\item {\bf \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model does not separate abilities from progress:}
\citeauthor{andersen:85}'s (\citeyear{andersen:85}) reparameterized model does not separate the abilities $\alpha_{i,1}$ and $\alpha_{i,2}$ of individual $i$ at time $1$ and $2$ from the rate of progress $\lambda_{i,2}$ of individual $i$ between time $1$ and $2$,
but assumes that the rate of progress $\lambda_{i,2} =  1 - \alpha_{i,2}\, /\, \alpha_{i,1}$ is a function of the abilities $\alpha_{i,1}$ and $\alpha_{i,2}$.
By contrast,
the latent process model separates the ability $\alpha_i$ of individual $i$ from the rate of progress $\lambda_{i,2}$ of individual $i$ between time $1$ and $2$.
}
\end{enumerate}
The simulations in Section \ref{sec:interaction} and the applications in Sections \ref{sec:depression} and \ref{sec:math} demonstrate the advantages of the interaction map provided by the latent process model over the one-dimensional ability map provided by \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model.


==> diff.logit.old.tex <==
For example,
one can assess whether individual $i$ makes more progress during some periods than others by inspecting changes in the linear predictors $\eta_{i,j,t}$.
To demonstrate,
consider binary responses $Y_{i,j,t} \in \{0, 1\}$ at times $t \in \{2, 3, 4\}$,
and assume that $Y_{i,j,t} \mid \mu_{i,j,t}\, \ind\, \mbox{Bernoulli}(\mu_{i,j,t})$ with log odds
\beno
\eta_{i,j,t}
&=&
\log \dfrac{\mu_{i,j,t}}{1-\mu_{i,j,t}}
&=& \begin{cases}
\alpha_i + \beta_j - d(\bm{a}_{i,2}, \mT)
& \mbox{if $t=2$}
\\
\alpha_i + \beta_j - d(\bm{a}_{i,3}, \mT)
& \mbox{if $t=3$}
\\
\alpha_i + \beta_j - d(\bm{a}_{i,4}, \mT)
& \mbox{if $t=4$,}
\end{cases}
\ee
assuming $\gamma=1$ to streamline comparisons.
The rate of progress of individual $i$ between time $2$ and $3$ and between time $3$ and $4$ can then be compared by comparing the changes of log odds between time $2$ and $3$ and between time $3$ and $4$:
\beno
\eta_{i,j,3} - \eta_{i,j,2}
&=& d(\bm{a}_{i,3}, \mT) - d(\bm{a}_{i,2}, \mT)\s
\\
\eta_{i,j,4} - \eta_{i,j,3}
&=& d(\bm{a}_{i,4}, \mT) - d(\bm{a}_{i,3}, \mT).
\ee
If,
e.g.,
\beno
d(\bm{a}_{i,3}, \mT) - d(\bm{a}_{i,2}, \mT)
&>& d(\bm{a}_{i,4}, \mT) - d(\bm{a}_{i,3}, \mT),
\ee
then individual $i$ makes more progress between time 2 and 3 than between time 3 and 4.


==> figure/advantages.metric.space.tex <==
The fact that individuals are embedded in the same metric space as the target helps capture
\bi
\item interactions between individuals and variables arising from unobserved variables,
such as cultural background, 
upbringing and mentoring of students,
which may affect responses;
\item whether individuals make progress towards the target;
\item how much progress individuals make towards the target;
\item whether individuals make more progress during some periods than others;
\item how much more progress individuals can make in the future.
\ei
We show, 
with the help of simulations and applications, 
that the latent process model enables a novel look at mental health and online educational assessments in disadvantaged subpopulations,
as demonstrated by the motivating example in Section \ref{example}.


==> figure/andersen.comparison.tex <==
\begin{figure}[htb]
    \centering
    \begin{tabular}{cc}
     G1 &  G2  \\
 \includegraphics[width=0.35 \textwidth]{figure/two_groups_test1.pdf}
  &   \includegraphics[width=0.35 \textwidth]{figure/two_groups_test2.pdf} \\
       \end{tabular}
\caption{Latent process model: The estimated interaction maps $(\mathbb{M}, d)$ with $\mathbb{M} \coloneqq \mR^2$ show the progress of four selected members of groups G1 (left) and G2 (right) towards target $\mT$.
Members of group G1 provided correct responses to variables 1--5 at time $1$ and variables 1--10 at time $2$,
while members of G2 provided correct responses to variables 16--20 at time $1$ and variables 11--20 at time $2$.
The estimated interaction maps reveal these group-variable interactions.
}
    \label{fig:progress1}
\end{figure}

To demonstrate that the latent process model can capture interactions between individuals and variables while \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model does not,
we consider $n = 200$ individuals divided into two groups G1 and G2 of the same size,
with the same progress but distinct responses to $p = 20$ variables.
Members of group G1 provide correct responses to variables 1--5 at time $1$ and variables 1--10 at time $2$,
while members of G2 provide correct responses to variables 16--20 at time $1$ and variables 11--20 at time $2$.
Both groups G1 and G2 make the same progress,
by increasing the number of correct responses from 5 to 10 between time $1$ and $2$,
but exhibit distinct response patterns.

\begin{figure}[htb]
    \centering 
    \begin{tabular}{cc} 
    G1 &  G2  \\
 \includegraphics[width=0.35 \textwidth]{figure/two_groups_andersen1.pdf}
  &   \includegraphics[width=0.35 \textwidth]{figure/two_groups_andersen2.pdf} \\

       \end{tabular}
\caption{\citeauthor{andersen:85}'s (\citeyear{andersen:85}) model:
The estimated progress of selected members of groups G1 (left) and G2 (right),
which are identical to the members of groups G1 and G2 in Figure \ref{fig:progress1}.
The vertical axis represents posterior means of $\alpha_{i,t}$.
Members of group G1 provided correct responses to variables 1--5 at time $1$ and variables 1--10 at time $2$,
while members of G2 provided correct responses to variables 16--20 at time $1$ and variables 11--20 at time $2$.
The estimated progress maps reveal that all group members make similar progress,
but do not reveal the group-variable interactions.
}
    \label{fig:progress2}
\end{figure}

Figure \ref{fig:progress1} shows estimated interaction maps $\mathbb{M} \coloneqq \mR^2$ of four selected members of groups G1 (left) and G2 (right).
These interaction maps reveal that the members of group G1 are located in a neighborhood of variables 1--5 at time $1$,
while the members of group G2 are located in a neighborhood of variables 16--20 at time $1$.
The placements of groups G1 and G2 aligns with the response patterns of groups G1 and G2.

We compare the results in Figure \ref{fig:progress1} to the results based on \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model.
The posterior means of abilities $\alpha_{i,t}$ of \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model with $\logit(\mu_{i,j,t}) = \alpha_{i,t} + \beta_j$ are shown in Figure \ref{fig:progress2}.
% estimated by the statistical software {\tt NIMBLE} \citep{nimble}.
% estimated by using a fully Bayesian approach with 5,000 iterations after 15,000 burn-in period. 
Figure \ref{fig:progress2} suggests that the selected members of groups G1 and G2 make similar progress,
but obscures the fact that the response patterns of groups G1 and G2 are distinct.
In other words,
\citeauthor{andersen:85}'s (\citeyear{andersen:85}) model does not capture interactions between individuals and variables.


==> figure/andersen.tex <==
A classic approach to measuring progress of students in educational assessments is based on \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model.

\citeauthor{andersen:85}'s (\citeyear{andersen:85}) model assumes that binary responses $Y_{i,j,t} \in \{0, 1\}$ are independent $\mbox{Bernoulli}(\mu_{i,j,t})$ random variables with log odds
\beno
\eta_{i,j,t}
&=& \log \dfrac{\mu_{i,j,t}}{1-\mu_{i,j,t}}
&\coloneqq& \alpha_{i,t} + \beta_j.
\ee
To compare \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model with the latent process model,
consider binary responses $Y_{i,j,t} \in \{0, 1\}$ by students $i$ to items $j$ at $T = 2$ time points $t \in \{1, 2\}$ along with the following reparameterization of \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model:
\beno
\alpha_{i,1} \;\;\coloneqq\;\; -\gamma\, d(\bm{a}_{i,1},\, \mT)\s
\\
\alpha_{i,2}
\;\;\coloneqq\;\; -\gamma\, d(\bm{a}_{i,2},\, \mT)
\;\;=\;\; -\gamma\, (1 - \lambda_{i,2})\, d(\bm{a}_{i,1},\, \mT)
\;\;=\;\; (1 - \lambda_{i,2})\; \alpha_{i,1},
\ee
where $\gamma \in [0, +\infty)$,
$d(\bm{a}_{i,t}, \mT) \coloneqq |\!|\bm{a}_{i,t} - \mT|\!|_2$ ($t \in \{1, 2\}$),
and $d(\bm{a}_{i,2},\, \mT) = (1 - \lambda_{i,2})\; \alpha_{i,1}$ by Equation \eqref{d.reduction} in Section \ref{special.cases}.

Then,
under \citeauthor{andersen:85}'s (\citeyear{andersen:85}) reparameterized model,
the rate of progress $\lambda_{i,2}$ of student $i$ between time $1$ and $2$ is a function of the distances $d(\bm{a}_{i,1},\, \mT)$ and $d(\bm{a}_{i,2},\, \mT)$:
\beno
\lambda_{i,2}
&=& 1 - \dfrac{\alpha_{i,2}}{\alpha_{i,1}}
&=& 1 - \dfrac{d(\bm{a}_{i,2},\, \mT)}{d(\bm{a}_{i,1},\, \mT)},
\ee
provided that $d(\bm{a}_{i,1},\, \mT) > 0$.
As a result,
\bi
\item the abilities $\alpha_{i,1}$ and $\alpha_{i,2}$ of student $i$ at time $1$ and $2$ can be interpreted in terms of distances $d(\bm{a}_{i,1},\, \mT)$ and $d(\bm{a}_{i,2},\, \mT)$ between student $i$ and learning target $\mT$ in an underlying metric space $(\mathbb{M},\, d)$,\vspace{.1cm}
\item $1 - \alpha_{i,2}\, / \alpha_{i,1}$ can be interpreted as the rate of progress of student $i$ towards learning target $\mT$.
\ei

That being said,
\citeauthor{andersen:85}'s (\citeyear{andersen:85}) model has two limitations:\vspace{.1cm}
\begin{enumerate}
\item {\bf \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model does not capture interactions:} 
\citeauthor{andersen:85}'s (\citeyear{andersen:85}) model assumes that the log odds
\beno
\eta_{i,j,t}
&=& \log \dfrac{\mu_{i,j,t}}{1-\mu_{i,j,t}}
&\coloneqq& \alpha_{i,t} + \beta_j
\ee
is additive in the ability $\alpha_{i,t}$ of student $i$ at time $t$ and the easiness $\beta_j$ of item $j$ and therefore cannot capture interactions between students $i$ and items $j$ arising from unobserved variables,
such as cultural background, upbringing, and mentoring.
As a result,
the underlying metric space $(\mathbb{M},\, d)$ of \citeauthor{andersen:85}'s (\citeyear{andersen:85}) reparameterized model cannot be interpreted as an interaction map,
but should be interpreted as an ability map:
In fact,
the distances $d(\bm{a}_{i,1},\, \mT) = -\alpha_{i,1}\, /\, \gamma \propto -\alpha_{i,1} \in [0,\, +\infty)$ and $d(\bm{a}_{i,2},\, \mT) = -\alpha_{i,2}\, /\, \gamma \propto -\alpha_{i,2} \in [0,\, +\infty)$ of individual $i$ to target $\mT$ at time $1$ and $2$ are proportional to the abilities $\alpha_{i,1}$ and $\alpha_{i,2}$.
By contrast,
the latent process model assumes that the log odds is
\beno
\eta_{i,j,t}
&=& \log \dfrac{\mu_{i,j,t}}{1-\mu_{i,j,t}}
&\coloneqq&
\begin{cases}
\alpha_i + \beta_j - \gamma\; d(\bm{a}_{i,1}, \bm{b}_j)
& \mbox{if } t = 1\s
\\
\alpha_i + \beta_j - \gamma\; (1 - \lambda_{i,2})\, d(\bm{a}_{i,1}, \mT)
& \mbox{if } t = 2,
\end{cases}
\ee
where $d(\bm{a}_{i,2},\, \mT) = (1 - \lambda_{i,2})\; \alpha_{i,1}$ by Equation \eqref{d.reduction} in Section \ref{special.cases}
As a consequence,
the latent process model can capture interactions between individuals (e.g., students) and variables (e.g., items):
e.g.,
in educational assessments,
a large distance between student $i$ and item $j$ indicates that the probability of a correct response of student $i$ to item $j$ is lower than would be expected based on the potential (ability) $\alpha_i$ of student $i$ and the easiness $\beta_j$ of item $j$.
Thus,
the underlying metric space $(\mathbb{M},\, d)$ of the latent process model should be interpreted as an interaction map rather than an ability map.
A simulation study in Section \ref{sec:interaction} confirms that the latent process model can capture interactions between students and items,
whereas \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model does not capture interactions.\vspace{.1cm}
\item {\bf \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model provides one-dimensional ability maps:}
The fact that the metric space $(\mathbb{M},\, d)$ underlying \citeauthor{andersen:85}'s (\citeyear{andersen:85}) reparameterized model represents an ability map gives rise to an additional limitation of \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model:
If,
e.g.,
$\mathbb{M} \coloneqq \mR^q$ ($q \geq 1$) and $d(\bm{a}_{i,t}, \mT) \coloneqq |\!|\bm{a}_{i,t} - \mT|\!|_2$,
then $q=1$ dimension is sufficient for representing the distances $d(\bm{a}_{i,t}, \mT)$ between individuals $i$ at time $t$ and learning target $\mT$ in $(\mathbb{M},\, d)$.
A Euclidean space $\mR^q$ of dimension $q \geq 2$ would provide a less parsimonious representation than $q = 1$ and therefore $q = 1$ is preferable to $q \geq 2$ according to Occam's razor \citep{JeBe92}.
By contrast,
the metric space $(\mathbb{M},\, d)$ underlying the latent process model represents an interaction map rather than an ability map.
To capture interactions between students and items,
a Euclidean space $\mR^q$ of dimension $q \geq 2$ may be required.
% The applications in Sections \ref{sec:depression} and \ref{sec:math} demonstrate that.
\hide{
\item {\bf \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model does not separate abilities from progress:}
\citeauthor{andersen:85}'s (\citeyear{andersen:85}) reparameterized model does not separate the abilities $\alpha_{i,1}$ and $\alpha_{i,2}$ of individual $i$ at time $1$ and $2$ from the rate of progress $\lambda_{i,2}$ of individual $i$ between time $1$ and $2$,
but assumes that the rate of progress $\lambda_{i,2} =  1 - \alpha_{i,2}\, /\, \alpha_{i,1}$ is a function of the abilities $\alpha_{i,1}$ and $\alpha_{i,2}$.
By contrast,
the latent process model separates the ability $\alpha_i$ of individual $i$ from the rate of progress $\lambda_{i,2}$ of individual $i$ between time $1$ and $2$.
}
\end{enumerate}
The simulations in Section \ref{sec:interaction} and the applications in Sections \ref{sec:depression} and \ref{sec:math} demonstrate the advantages of the interaction map provided by the latent process model over the one-dimensional ability map provided by \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model.


==> figure/aoas_revision_analysis.tex <==
\section{Simulations}
\label{sec:simulations}

\alert{We conduct two simulation studies: 
\bi
\item In Section \ref{sec:misspecification}, 
we investigate whether the proposed statistical framework can capture interesting features of real-world data that have not been generated by the model.
In other words, 
we investigate the behavior of the proposed statistical framework under model misspecification.\vspace{.1cm}
\item In Section \ref{sec:interaction}, 
we demonstrate how the proposed model can capture interactions between individuals and variables,
whereas \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model does not.
\ei
}

Throughout Sections \ref{sec:simulations},  
\ref{sec:depression}, 
and \ref{sec:math},
we focus on binary responses $Y_{i,j,t} \in \{0, 1\}$ at $T = 2$ time points $t \in \{1, 2\}$ and write $\lambda_i$ instead of $\lambda_{i,2}$.
All results are based on the proposed latent process model with a logit link function and the special case $\mathbb{M} \coloneqq \mR^q$ and $d(\bm{a}_{i,t}, \mT) \coloneqq |\!|\bm{a}_{i,t} - \mT|\!|_2$.
The prior and Markov chain Monte Carlo algorithm are described in Supplement \ref{appendix:estimation}.

\hide{
For Study 1, we compare results based on $\mathbb{M} \coloneqq \mR$,\, $\mR^2$, $\mR^3$, and $\mR^4$ using the Watanabe–Akaike information criterion \citep{waic} along with interaction maps based on $\mR$,\, $\mR^2$, and $\mR^3$. 
\textcolor{blue}{For Study 2, we focus on $\mathbb{M} \coloneqq \mR^2$ for the sake of simplicity. }
}

\subsection{Simulation Study I: Model Misspecification}\label{sec:misspecification}

\subsubsection{Scenario $n=300$, $p=10$, $T=2$} 
\label{sec:sim_scenario1}

\begin{table}[htb]
    \centering
    \begin{tabular}{l|cccr}
    \hline 
$\mathbb{M}$  & 10\% Percentile & Median & 90\% Percentile & Minimizer of WAIC\\
      \hline 
$\mathbb{M} \coloneqq \mR$ & 17937& 18170& 19228  & 2.0\% \\ 
$\mathbb{M} \coloneqq \mR^2$ & 17639& 17815& 18016 & 73.2\%   \\
$\mathbb{M} \coloneqq \mR^3$ & 17613& 18129& 18391  & 21.6\% \\
$\mathbb{M} \coloneqq \mR^4$ &18075& 18304& 18512  &  3.2\% \\
\hline
\end{tabular}
\caption{Simulation results ($n = 300$):
Watanabe–Akaike information criterion (WAIC) based on 250 simulated data sets.
The last column indicates how often the latent process model with $\mathbb{M} \coloneqq \mR$,\, $\mR^2$, $\mR^3$, $\mR^4$ minimized the WAIC. 
}
\label{tab:sim2_fit}
\end{table}

We first consider a scenario in which the progress of individuals towards a target of interest $\mT \in \mathbb{M} \coloneqq \mR^q$ is assessed based on binary responses $Y_{i,j,t} \in \{0, 1\}$ of $n = 300$ individuals to $p=10$ variables at $T = 2$ time points $t \in \{1, 2\}$.
We assume that there are three groups of individuals,
called G1, G2, and G3.
Each group is comprised of 100 individuals. 
At time 1,
the success probabilities of all individuals are .2.
At time 2, 
individuals have success probabilities .25 (G1), .5 (G2), and .75 (G3).  
We generated 250 data sets and estimated the latent process model with $\mathbb{M} \coloneqq \mR^q$ and $q \in \{1, 2, 3, 4\}$. 
\textcolor{blue}{The resulting interaction maps of those three groups of individuals are presented in Supplement \ref{appendix:add}.}

The Watanabe–Akaike information criterion \citep{waic} in Table \ref{tab:sim2_fit} suggests that the latent process model with $\mathbb{M} \coloneqq \mR^2$ is more adequate than $\mathbb{M} \coloneqq \mR$,\,
$\mR^3$,
and $\mR^4$.

A natural question to ask is whether the latent process model can separate groups G1, G2, and G3 based on data.
Figure \ref{fg:sim2_progress} indicates that the latent process model with $\mathbb{M} \coloneqq \mR^q$ and $q \in \{1, 2, 3\}$ can distinguish groups G1, G2, and G3,
despite the fact that the data were not generated by the model. 
That said,
the latent process model with $\mathbb{M} \coloneqq \mR^2$ or $\mR^3$ can better distinguish groups G1, G2, and G3 than the latent process model with $\mathbb{M} \coloneqq \mR$,
reinforcing the findings in Table \ref{tab:sim2_fit}.

A related question is whether the latent process model can distinguish individuals with non-neglible progress from those with negligible progress,
based on the two-component mixture prior for the rates of progress $\lambda_i$ of individuals $i$ described in Section \ref{sec:prior}.
Figure \ref{fg:sim2_count} reveals that---among the 100 individuals in groups G1, G2, and G3---the percentage of individuals deemed to have made negligible progress is more than 80\% in the low-progress group G1;
is between 40\% and 80\% in the moderate-progress group G2;
and is less than 20\% in the high-progress group G3.
The latent process model with $\mathbb{M} \coloneqq \mR^2$ or $\mR^3$ seems to lead to more accurate assessments,
compared with the latent process model with $\mathbb{M} \coloneqq \mR$.

\begin{figure}[htbp]
\begin{tabular}{cccc}
$\mathbb{M} \coloneqq \mR$ & $\mathbb{M} \coloneqq \mR^2$ & $\mathbb{M} \coloneqq \mR^3$\\
     \includegraphics[width=.31\textwidth]{figure/sim_small2_la_1d.pdf} 
     &
 \includegraphics[width=.31\textwidth]{figure/sim_small2_la_2d.pdf} 
 &
      \includegraphics[width=.31\textwidth]{figure/sim_small2_la_3d.pdf} 
     \\
 \end{tabular}
\caption{\alert{Simulation results ($n = 300$): Histogram of the mean of 100 posterior medians of the rates of progress $\lambda_i$ of individuals $i$ in groups G1, G2, G3 across 250 data sets.}}
\label{fg:sim2_progress}
\end{figure}

\begin{figure}[htbp]
    \centering
\begin{tabular}{cccc}
$\mathbb{M} \coloneqq \mR$ & $\mathbb{M} \coloneqq \mR^2$ & $\mathbb{M} \coloneqq \mR^3$\\ 
     \includegraphics[width=.31\textwidth]{figure/sim_small2_pi_1d_sum_v2.pdf} 
     %\includegraphics[width=.31\textwidth]{figure/sim_small2_pi_1d_sum.pdf} 
     &
 \includegraphics[width=.31\textwidth]{figure/sim_small2_pi_2d_sum.pdf} 
&
    \includegraphics[width=.31\textwidth]{figure/sim_small2_pi_3d_sum.pdf}    
     \\
 \end{tabular}
\caption{Simulation results ($n = 300$):
Boxplots of the number of individuals in groups G1, G2, G3 deemed to have made negligible progress.}
\label{fg:sim2_count}
\end{figure}

\subsubsection{Scenario $n=600$, $p=10$, $T=2$}
\label{sec:sim_scenario2}

\begin{table}[htb]
    \centering
    \begin{tabular}{l|cccr}
    \hline 
$\mathbb{M}$  & 10\% Percentile & Median & 90\% Percentile & Minimizer of WAIC\\

      \hline 
$\mathbb{M} \coloneqq \mR$ & 35703 & 36567& 38665   & 10.0\% \\ 
$\mathbb{M} \coloneqq \mR^2$ & 35256 &35567 &35920  & 79.6\%  \\
$\mathbb{M} \coloneqq \mR^3$ & 35581 &36017 &36639  & 10.4\%   \\
$\mathbb{M} \coloneqq \mR^4$ & 36243 &36976 &38083   & 0.0\%   \\
\hline
    \end{tabular}
\caption{Simulation results ($n = 600$):
Watanabe–Akaike information criterion (WAIC) based on 250 simulated data sets.
The last column indicates how often the latent process model with $\mathbb{M} \coloneqq \mR$,\, $\mR^2$, $\mR^3$, $\mR^4$ minimized the WAIC. 
}
    \label{tab:sim3_fit}
\end{table}

We double the sample size from $n = 300$ to $n = 600$ to explore the behavior of the latent process model as the sample size increases.
We assume that there are four groups of individuals,
called G1, G2, G3 and G4.
Each group is comprised of 150 individuals. 
At time 1 the success probabilities of all individuals are .2, 
while at time 2 individuals have success probabilities .3 (G1), .5 (G2), .7 (G3), and .9 (G4). 
We generated 250 data sets and estimated the latent process model with $\mathbb{M} \coloneqq \mR^q$ and $q \in \{1, 2, 3, 4\}$. 
\textcolor{blue}{The resulting interaction maps of those three groups of individuals are presented in Supplement \ref{appendix:add}.}

\begin{figure}[t]
    \centering
\begin{tabular}{cccc}
$\mathbb{M} \coloneqq \mR$ & $\mathbb{M} \coloneqq \mR^2$ & $\mathbb{M} \coloneqq \mR^3$\\ 
     \includegraphics[width=.31\textwidth]{figure/sim_small33_la_1d.pdf} 
     &
 \includegraphics[width=.31\textwidth]{figure/sim_small33_la_2d.pdf} 
 &
 \includegraphics[width=.31\textwidth]{figure/sim_small33_la_3d.pdf}      
     \\
 \end{tabular}
\caption{Simulation results ($n = 600$):
Histogram of the posterior medians of the rates of progress $\lambda_i$ of individuals $i$ in groups G1, G2, G3, G4.
}
\label{fg:sim3_progress}
\end{figure}

The results dovetail with the results in Section \ref{sec:sim_scenario1},
but suggest that the one-dimensional space $\mathbb{M} \coloneqq \mR$ is even less appealing when $n$ is large:
First, 
the Watanabe–Akaike information criterion \citep{waic} in Table \ref{tab:sim3_fit} favors $\mathbb{M} \coloneqq \mR^2$ over $\mR$,\, $\mR^3$, and $\mR^4$.
Second,
the latent process model can distinguish the groups G1, G2, G3, and G4 when $\mathbb{M} \coloneqq \mR^q$ and $q \geq 2$ according to Figure \ref{fg:sim3_progress},
but the groups G1, G2, G3, and G4 are less well-separated when $\mathbb{M} \coloneqq \mR$.

{\color{blue} 
\subsection{Simulation Study II: Interactions}
\label{sec:interaction}

\input{andersen.comparison.tex}

}

\section{Application: mental health}
\label{sec:depression}

We describe the motivating example introduced in Section \ref{example} in more detail. 
The motivating example is concerned with assessing the progress of vulnerable population members in terms of mental health.
We focus on a vulnerable population of special interest:
mothers with infants in low-income communities.

\subsection{Data}
\label{sec:mental.health.data}

\cite{santos:18} conducted between 2003 and 2010 large-scale randomized clinical trials in low-income communities in the U.S.\ states of North Carolina and New York \citep{beeber:14}. 
% The control group received either usual care or equal attention and healthy education condition. 
The data set consists of 306 low-income mothers with infants aged 6 weeks to 36 months,
enrolled in the Early Head Start Program in North Carolina or New York. 
The mental health of these mothers was assessed four times (baseline, 14 weeks, 22 weeks, and 26 weeks).
We focus on the $n = 257$ mothers who participated in the first two assessments. 
% These $n = 257$ mothers were assigned to two groups:
% a treatment group and a control group.
% The treatment focused on decreasing maternal depressive symptoms through interpersonal psychotherapy and parent enhancement intervention. 
The Center for Epidemiological Studies Depression (CES-D) scale was used to measure depression of the mothers.
We focus on $p=10$ items:
1 (``bothered"), 
2 (``trouble in concentration"), 
3 (``feeling depressed"), 
4 (``effort"), 
5 (``not feeling hopeful"), 
6 (``failure"), 
7 (``not happy"), 
8 (``talking less"), 
9 (``people dislike"), 
and 10 (``get going"),
described in Supplement \ref{depression_items}. 
To measure progress toward the target of interest (improving mental health),
we recoded the $p=10$ items by assigning ``depression" $\mapsto$ 0 and ``no depression" $\mapsto$ 1.  
The proportions of positive responses (``no depression") range from .436 to .747 at the pre-assessment (median .630), 
and from .621 to .859 at the post-assessment (median .777). 

%Descriptive statistics are presented in Table \ref{tab:ces-d}. % with descriptive statistics. 

%The Center for Epidemiological Studies Depression (CES-D) scale was used to measure depression severity at four time points and we focused on the first two assessments. % at baseline (T1-first intervention session), 14 weeks (T2- second intervention session), and 22 weeks (T3- one month after intervention completion), and 26 weeks post-baseline (T4-one month after intervention completion). 
 % ($n$=153 in treatment and n=151 in control groups). 
%In this study we focused on the first two assessment We included 257 mothers who completed the first two surveys in the data. 
%We focused on 16 depressive symptoms. %Four symptoms were excluded that behave somewhat differently from the other symptoms. These include:  (3) Feeling blue; (4) Lack of feeling good; (11) Sleep disturbances; (16) Lack of enjoyment). 

\subsection{Results}
\label{sec:dep_spike}

\begin{table}[tbh]
    \centering
    \begin{tabular}{l|cccr}
$\mathbb{M}$  & Minimum & Median & Maximum & Minimizer of WAIC\\
      \hline  
$\mathbb{M} \coloneqq \mR$ & 14650      &14713    & 14897 & 0\% \\ 
$\mathbb{M} \coloneqq \mR^2$ & 14432    & 14606  &  14679 & 0\%   \\
$\mathbb{M} \coloneqq \mR^3$ & 14351   & 14450    & 14509 & 100\% \\
$\mathbb{M} \coloneqq \mR^4$ & 14499   & 14623    & 14741 & 0\% \\
\hline
    \end{tabular}
\caption{Mental health: 
Watanabe–Akaike information criterion (WAIC) based on five Markov chain Monte Carlo runs.
The last column indicates how often the latent process model with $\mathbb{M} \coloneqq \mR$,\, $\mR^2$, $\mR^3$, $\mR^4$ minimized the WAIC. 
}
    \label{tab:waic_dep}
\end{table}
We assess the progress of $n = 257$ low-income mothers towards the target of interest $\mT$ (improving mental health),
measured by $p = 10$ items.
The priors and Markov chain Monte Carlo algorithm can be found in Supplement \ref{appendix:estimation}.
To detect signs of non-convergence,
we used trace plots along with the multivariate Gelman-Rubin potential scale reduction factor of \citet{vats:18a}.
These convergence diagnostics are reported in Supplement \ref{appendix:convergence} and do not reveal signs of non-convergence.

Table \ref{tab:waic_dep} shows the Watanabe–Akaike information criterion \citep{waic} based on the latent process model with $\mathbb{M} \coloneqq \mR^q$ and $q \in \{1, 2, 3, 4\}$,
suggesting that $\mathbb{M} \coloneqq \mR^3$ is most appropriate.

\begin{figure}[htbp]
    \centering
\begin{tabular}{ccc}
$\mathbb{M} \coloneqq \mR$ & $\mathbb{M} \coloneqq \mR^2$ & $\mathbb{M} \coloneqq \mR^3$ \\ 
     \includegraphics[width=.31\textwidth]{figure/dep_one_4_poly_spike_1d_1_sharp.pdf} 
     &  \includegraphics[width=.31 \textwidth]{figure/dep_one_4_poly_spike_2d_1_sharp.pdf} 
     &  \includegraphics[width=.31 \textwidth]{figure/dep_one_4_poly_spike_3d_1_sharp_v2.png}  
   % &  \includegraphics[width=.31 \textwidth]{figure/dep_one_4_poly_spike_3d_1_sharp.png}  
     \\
\end{tabular}
\caption{Mental health: 
Interaction maps $(\mathbb{M},\, d)$ with $\mathbb{M} \coloneqq \mR^q$ and $q \in \{1, 2, 3\}$ show the progress of low-income mothers $A$, $B$, $C$, $D$ towards target $\mT$ (improving mental health),
measured by items $1, \dots, 10$ (questions about depression).
The positions of mothers and items are estimated by posterior medians.
While the one-dimensional interaction map ($q=1$) suggests that all items are close to target $\mT$, 
the three-dimensional interaction map ($q = 3$) reveals interactions between mothers and items:
e.g.,
item $5$ deviates from the bulk of the items,
and mother $B$ is closest to item $5$.
It turns out that mother $B$ agreed with item $5$ at the first assessment (``feeling hopeful"),
whereas mothers $A$, $C$, $D$ did not.
In addition,
the interaction map suggests that mothers $B$ and $C$ have made strides towards improving mental health,
whereas mothers $A$ and $D$ may need to make more progress.
}
\label{fg:dep_progress2}
\end{figure}

\begin{figure}[htbp]
    \centering
\begin{tabular}{cccc}
$\mathbb{M} \coloneqq \mR$ & $\mathbb{M} \coloneqq \mR^2$ & $\mathbb{M} \coloneqq \mR^3$\\ 
        \includegraphics[width=.31 \textwidth]{figure/dep_kernel_poly_spike_1d_1_sharp.pdf}
     &  \includegraphics[width=.31 \textwidth]{figure/dep_kernel_poly_spike_2d_1_sharp.pdf}
     &  \includegraphics[width=.31 \textwidth]{figure/dep_kernel_poly_spike_3d_1_sharp.pdf}
     \\
\end{tabular}
\caption{Mental health:
Marginal posteriors of the rates of progress $\lambda_A$, $\lambda_B$, $\lambda_C$, $\lambda_D$ of mothers $A$, $B$, $C$, $D$ towards target $\mT$ (improving mental health).
The progress of mother $A$ is unclear,
but the marginal posteriors of the rates of progress $\lambda_B$ and $\lambda_C$ of mothers $B$ and $C$ have modes close to $1$,
confirming that mothers $B$ and $C$ have made strides towards improving mental health.
By contrast,
the mode of the marginal posterior of the rate of progress $\lambda_D$ of mother $D$ is close to $0$,
suggesting that mother $D$ may need additional assistance.
}
\label{fg:dep_kernel2}
\end{figure}
We present interaction maps in Figure \ref{fg:dep_progress2}.
While the one-dimensional interaction map suggests that all items are close to target $\mT$, 
the three-dimensional interaction map (which, according to the Watanabe–Akaike information criterion, is more appropriate than the one-dimensional interaction map) reveals that there are interactions between individuals (mothers) and items (questions about depression):
e.g.,
item $5$ deviates from the bulk of the items,
and mother $B$ is closest to item $5$.
It turns out that mother $B$ agreed with item $5$ at the first assessment (``feeling hopeful"),
whereas mothers $A$, $C$, and $D$ did not.
In addition,
the interaction map suggests that mothers $B$ and $C$ have made strides towards improving mental health,
whereas mothers $A$ and $D$ may need to make more progress in the future.

The posterior summaries in Table \ref{tab:dep_lambda} confirms that,
more likely than not,
mothers $B$ and $C$ have made progress,
while mother $D$ has not.
To gain more insight into the uncertainty about the progress of mothers $A$, $B$, $C$, and $D$, 
we present the marginal posteriors of $\lambda_A$,
$\lambda_B$,
$\lambda_C$,
and $\lambda_D$ in Figure \ref{fg:dep_kernel2}.
The marginal posteriors of $\lambda_A$,
$\lambda_B$,
$\lambda_C$,
and $\lambda_D$ caution that there is non-negligible uncertainty about the progress of some of the mothers.
A case in point is mother $A$:
The marginal posterior of mother $A$'s rate of progress $\lambda_A$ resembles the Uniform$(0, 1)$ distribution.
As a consequence, 
it is unclear whether mother $A$ has made progress,
and how much.
By contrast,
the marginal posteriors of the rates of progress $\lambda_B$ and $\lambda_C$ of mothers $B$ and $C$ have modes close to $1$,
suggesting that mothers $B$ and $C$ have made strides towards improving mental health.
The marginal posterior of the rate of progress $\lambda_D$ of mother $D$ has a mode close to $0$,
which underscores that mother $D$ may need additional assistance.

To assess the goodness-of-fit of the model,
we generated 1,000 posterior predictions of the proportions of positive responses at the second assessment.
Figure \ref{fg:dep_ppc} shows the proportions of predicted and observed positive responses. 
By and large, 
the model predictions agree with the observations.

\begin{figure}[htbp]
    \centering
\begin{tabular}{cccc}
$\mathbb{M} \coloneqq \mR$ & $\mathbb{M} \coloneqq \mR^2$ & $\mathbb{M} \coloneqq \mR^3$\\ 
     \includegraphics[width=.31\textwidth]{figure/dep_check_person_poly_spike_1d_1_sharp.pdf} 
     &  \includegraphics[width=.31 \textwidth]{figure/dep_check_person_poly_spike_2d_1_sharp.pdf} 
     &  \includegraphics[width=.31 \textwidth]{figure/dep_check_person_poly_spike_3d_1_sharp.pdf}  
     \\
\end{tabular}
\caption{Mental health: 
Posterior predictions of the proportions of positive responses by mothers $A$, $B$, $C$, $D$ at the second assessment.
The observed proportions are indicated by red circles.
}
\label{fg:dep_ppc}
\end{figure}

\begin{table}[tbh]
\begin{tabular}{c cccc}
 & 10\% Percentile & Median & 90\% Percentile & Probability: Progress? \\ 
  \hline
 $\mathbb{M} \coloneqq \mR$:  &&&& \\   
  $\lambda_A$ & .060 & .290 & .790 & .550 \\ 
  $\lambda_B$ & .085 & .578 & .950 & .707 \\ 
  $\lambda_C$ & .213 & .775 & .965 & .847 \\ 
  $\lambda_D$ & .041 & .179 & .517 & .415 \\  
    \hline
 $\mathbb{M} \coloneqq \mR^2$:  &&&& \\  
  $\lambda_A$ & .055 & .255 & .757 & .518 \\ 
  $\lambda_B$ & .092 & .590 & .946 & .718 \\ 
  $\lambda_C$ & .278 & .790 & .965 & .866 \\ 
  $\lambda_D$ & .039 & .147 & .463 & .377 \\ 
      \hline
 $\mathbb{M} \coloneqq \mR^3$:  &&&& \\ 
  $\lambda_A$ & .058 & .258 & .806 & .527 \\ 
  $\lambda_B$ & .090 & .599 & .944 & .718 \\ 
  $\lambda_C$ & .280 & .774 & .969 & .861 \\ 
  $\lambda_D$ & .038 & .148 & .464 & .385 \\ 
      \hline
\end{tabular}
\caption{Mental health: 
Marginal posteriors of the rates of progress $\lambda_A$, $\lambda_B$, $\lambda_C$, $\lambda_D$ of mothers $A$, $B$, $C$, $D$.
The last column (``Probability: Progress?") shows the posterior probability of non-negligible progress.
}
\label{tab:dep_lambda}
\end{table}

\section{Application: online educational assessments}
\label{sec:math}

We present an application to online educational assessments, 
using the My Math Academy data \citep{bang:22}.

\begin{figure}[hptb]
\centering
\includegraphics[scale = .325]{figure/question24.png}
\includegraphics[scale = .325]{figure/question25.png}
\includegraphics[scale = .325]{figure/question30.png}
\\
\caption{\label{fig:math_academy0}
My Math Academy: 
Selected questions 24, 25, 30 corresponding to items 6, 7, 8.
Each question has a single correct response.
Items 6, 7, 8 are indicators of whether students choose the correct response to questions 24, 25, 30.
}
\end{figure}

\subsection{Data}

The My Math Academy data set consists of 479 kindergarten children, first- and second-grade students who participated in the My Math Academy effectiveness study in 2019 \citep{bang:22}. 
The students worked on pre- and post-assessments before and after working on the online learning platform My Math Academy. 
The pre- and post-assessments were separated by three months,
and both included a common set of 31 problems.
% The post-assessment included an additional set of seven problems, 
% but students were instructed not to solve them if the problems turned out to be too challenging.
We focus on $p = 8$ items measuring numerical understanding. 
Three selected items are presented in Figure \ref{fig:math_academy0}.
We exclude 58 of the 479 children who had no responses at either the pre- or post-assessment or who reported no background information. 
55\% of the remaining $n = 421$ students are kindergarten children,
48\% are female, 
87\% are low-income students eligible to receive free lunches, 
87\% are Hispanic, 
and 6\% are African-American. 
The proportions of correct responses range from .114 to .556 at the pre-assessment (median .397),
and from .216 to .755 at the post-assessment (median .544).

\subsection{Results}
\label{sec:math_spike}

\begin{table}[tbh]
    \centering
    \begin{tabular}{l|cccr}
$\mathbb{M}$  & Minimum & Median & Maximum & Minimizer of WAIC\\
      \hline  
$\mathbb{M} \coloneqq \mR$ & 20209 & 20310  & 20597  & 0\% \\ 
$\mathbb{M} \coloneqq \mR^2$ &  19838  &  20035  & 20077 & 60\%   \\
$\mathbb{M} \coloneqq \mR^3$ &  19841   & 20032  & 20071 & 40\%  \\
$\mathbb{M} \coloneqq \mR^4$ &   20166  & 20436  &  20678 & 0\%  \\
\hline
    \end{tabular}
\caption{My Math Academy: 
Watanabe–Akaike information criterion (WAIC) based on five Markov chain Monte Carlo runs.
The last column indicates how often the latent process model with $\mathbb{M} \coloneqq \mR$,\, $\mR^2$, $\mR^3$, $\mR^4$ minimized the WAIC. 
}
    \label{tab:waic_math}
\end{table}

We assess the progress of $n = 421$ students towards the target of interest (numerical understanding),
measured by $p = 8$ items.
The prior and Markov chain Monte Carlo algorithm are described in Supplement \ref{appendix:estimation}.
To detect signs of non-convergence,
we used trace plots along with the multivariate Gelman-Rubin potential scale reduction factor of \citet{vats:18a}.
These convergence diagnostics can be found in Supplement \ref{appendix:convergence} and do not reveal signs of non-convergence.

Table \ref{tab:waic_math} shows the Watanabe–Akaike information criterion \citep{waic} based on the latent process model with $\mathbb{M} \coloneqq \mR^q$ and $q \in \{1, 2, 3, 4\}$.
The Watanabe–Akaike information criterion suggests that $\mathbb{M} \coloneqq \mR^2$ or $\mR^3$ is most appropriate.

\begin{figure}[htbp]
    \centering
\begin{tabular}{ccc}
$\mathbb{M} \coloneqq \mR$ & $\mathbb{M} \coloneqq \mR^2$ & $\mathbb{M} \coloneqq \mR^3$\\ 
     \includegraphics[width=.31\textwidth]{figure/math_one_4_poly_spike_1d.pdf} 
     &  \includegraphics[width=.31 \textwidth]{figure/math_one_4_poly_spike_2d.pdf} 
     &  \includegraphics[width=.31 \textwidth]{figure/math_one_4_poly_spike_3d_v2.png}  
%    &  \includegraphics[width=.31 \textwidth]{figure/math_one_4_poly_spike_3d.png}  
     \\
\end{tabular}
\caption{My Math Academy: 
Interaction maps $(\mathbb{M},\, d)$ with $\mathbb{M} \coloneqq \mR^q$ and $q \in \{1, 2, 3\}$ show the progress of Hispanic students $A$, $B$, $C$, $D$ in low-income families towards learning target $\mT$ (numerical understanding),
measured by items $1, \dots, 8$. 
The positions of students and items are estimated by posterior medians.
While the one-dimensional interaction map ($q = 1$) suggests that all items are close to learning target $\mT$,
the two- and three-dimensional interaction maps ($q \in \{2, 3\}$) indicate that some of the items deviate from the bulk of the items:
e.g.,
item 6 is the most abstract item among the counting-related items 5, 6, 7 and the two- and three-dimensional interaction map reveal that item 6 deviates from learning target $\mT$ more than any other item.
Student $B$ is closest to item 6 and provided a correct response to item 6 at the pre-assessment,
whereas students $A$, $C$, $D$ did not.
}
\label{fg:math_progress}
\end{figure}

Figure \ref{fg:math_progress} shows interaction maps,
focusing on selected Hispanic students $A$, $B$, $C$, and $D$ in low-income families.
While the one-dimensional interaction map suggests that all items are close to learning target $\mT$,
the two- and three-dimensional interaction maps (which, according to the Watanabe–Akaike information criterion, are more appropriate than the one-dimensional interaction map) indicate that some of the items deviate from the bulk of the items:
e.g.,
item 6 is the most abstract item among the counting-related items 5, 6, and 7 and the two- and three-dimensional interaction map reveal that item 6 deviates from learning target $\mT$ more than any other item.
Student $B$ is closest to item 6 and provided a correct response to item 6 at the pre-assessment,
whereas students $A$, $C$, and $D$ did not.
\alert{\input{added.value.tex}}
% DO NOT DELETE:
% Student A was the one and only student with a correct response to item 6 at time 2.
% is the closest to item 6 and is indeed the only student how answered item 6 correctly at time $1$. 
% \textcolor{red}{[item 5,6,and 7 are all about counting to 100 by ones and tens. item 5 is given with pictures (multiple choice) , item 6 is only in words (multiple choice), and item 7 is given with some pictures (and drag and drop). item 5 is the easiest and item 6 is the most difficult. Student B is the only one who gets item 6 correct at time  1. At time 2, Student A is the only one who get items 6 right]}

Posterior summaries of the rates of progress $\lambda_A$, $\lambda_B$, $\lambda_C$, and $\lambda_D$ of students $A$, $B$, $C$, and $D$ are shown in Table \ref{tab:math_lambda}.
These posterior summaries confirm that,
with high posterior probability,
students $A$ and $D$ have made non-negligible progress,
but there is more uncertainty about students $B$ and $C$. 
To gain more insight into the uncertainty about the progress of students $A$, $B$, $C$, and $D$,
we present the marginal posteriors of the rates of progress $\lambda_A$, $\lambda_B$, $\lambda_C$, and $\lambda_D$ of students $A$, $B$, $C$, and $D$ in Figure \ref{fg:math_kernel}.
The marginal posteriors reveal non-negligible uncertainty:
e.g.,
the marginal posteriors of the rates of progress $\lambda_A$ and $\lambda_D$ of students $A$ and $D$ have modes close to $1$,
but both of them have long tails.
Assessing the progress of students $B$ and $C$ is harder still.

To assess the goodness-of-fit of the model,
we generated 1,000 posterior predictions of the proportions of correct responses at the post-assessment.
Figure \ref{fg:math_ppc} suggests that the posterior predictions by and large match the observed proportions of correct responses.

\begin{figure}[htbp]
    \centering
\begin{tabular}{cccc}
$\mathbb{M} \coloneqq \mR$ & $\mathbb{M} \coloneqq \mR^2$ & $\mathbb{M} \coloneqq \mR^3$\\ 
     \includegraphics[width=.31\textwidth]{figure/math_kernel_poly_spike_1d.pdf} 
     &  \includegraphics[width=.31 \textwidth]{figure/math_kernel_poly_spike_2d.pdf} 
     &  \includegraphics[width=.31 \textwidth]{figure/math_kernel_poly_spike_3d.pdf}  
     \\
\end{tabular}
\caption{My Math Academy:
Marginal posteriors of the rates of progress $\lambda_A$, $\lambda_B$, $\lambda_C$, $\lambda_D$ of Hispanic students $A$, $B$, $C$,$D$ towards learning target $\mT$ (numerical understanding).
}
\label{fg:math_kernel}
\end{figure}

\begin{figure}[htbp]
    \centering
\begin{tabular}{cccc}
$\mathbb{M} \coloneqq \mR$ & $\mathbb{M} \coloneqq \mR^2$ & $\mathbb{M} \coloneqq \mR^3$\\ 
     \includegraphics[width=.31\textwidth]{figure/math_check_person_poly_spike_1d.pdf} 
     &  \includegraphics[width=.31 \textwidth]{figure/math_check_person_poly_spike_2d.pdf} 
     &  \includegraphics[width=.31 \textwidth]{figure/math_check_person_poly_spike_3d.pdf}  
     \\
\end{tabular}
\caption{My Math Academy: 
Posterior predictions of the proportions of correct responses by Hispanic students $A$, $B$, $C$, $D$ at the post-assessment.
The observed proportions are indicated by red circles.
}
\label{fg:math_ppc}
\end{figure}

\begin{table}[ht]
\centering
\begin{tabular}{c cccc}
 & 10\% Percentile & Median & 90\% Percentile & Probability: Progress? \\ 
  \hline
$\mathbb{M} \coloneqq \mR$:  &&&& \\   
$\lambda_A$ & .196 & .817 & .970 & .863 \\ 
$\lambda_B$ & .072 & .419 & .918 & .635 \\ 
$\lambda_C$ & .055 & .246 & .826 & .523 \\ 
$\lambda_D$ & .107 & .648 & .953 & .743 \\ 
    \hline
$\mathbb{M} \coloneqq \mR^2$:  &&&& \\  
$\lambda_A$ & .352 & .837 & .970 & .900 \\ 
$\lambda_B$ & .080 & .424 & .913 & .642 \\ 
$\lambda_C$ & .051 & .250 & .814 & .515 \\ 
$\lambda_D$ & .116 & .653 & .948 & .770 \\ 
      \hline
$\mathbb{M} \coloneqq \mR^3$:  &&&& \\  
$\lambda_A$ & .322 & .814 & .970 & .885 \\ 
$\lambda_B$ & .076 & .406 & .920 & .634 \\ 
$\lambda_C$ & .051 & .227 & .771 & .498 \\ 
$\lambda_D$ & .133 & .639 & .947 & .765 \\ 
      \hline
\end{tabular}
\caption{My Math Academy: 
Summaries of the marginal posteriors of the rates of progress $\lambda_A$, $\lambda_B$, $\lambda_C$, $\lambda_D$ of students $A$, $B$, $C$, $D$.
The last column (``Probability: Progress?") shows the posterior probability of non-negligible progress.
}
\label{tab:math_lambda}
\end{table}



==> figure/diff.logit.tex <==
For example,
one can assess whether individual $i$ makes more progress during some periods than others by inspecting changes in the linear predictors $\eta_{i,j,t}$.
To demonstrate how one can assess whether individual $i$ makes more progress during some periods than others and to compare the proposed model to \citeauthor{andersen:85}'s (\citeyear{andersen:85}) classic model,
consider binary responses $Y_{i,j,t} \in \{0, 1\}$ at time $t \in \{2, 3, 4\}$ and assume that $Y_{i,j,t} \mid \mu_{i,j,t}\, \ind\, \mbox{Bernoulli}(\mu_{i,j,t})$ with log odds $\eta_{i,j,t}$.
To simplify the comparison,
we write henceforth $\mu_{i,j,t}$ and $\eta_{i,j,t}$ instead of $\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \bm{b}_j)$ and $\eta_{i,j,t}(\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \bm{b}_j))$,
respectively.

Under \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model with log odds
\beno
\eta_{i,j,t}
&=& \log\dfrac{\mu_{i,j,t}}{1-\mu_{i,j,t}} 
&=& 
\begin{cases}
\alpha_{i,2} + \beta_j & \mbox{ if $t=2$}
\\
\alpha_{i,3} + \beta_j & \mbox{ if $t=3$}
\\
\alpha_{i,4} + \beta_j & \mbox{ if $t=4$,}
\end{cases}
\ee
one can assess whether individual $i$ makes more progress between time $2$ and $3$ than between time $3$ and $4$ by inspecting changes in log odds:
\beno
\eta_{i,j,3} - \eta_{i,j,2} &=& \alpha_{i,3} - \alpha_{i,2}\s
\\
\eta_{i,j,4} - \eta_{i,j,3} &=& \alpha_{i,4} - \alpha_{i,3}.
\ee
If, 
e.g.,
\beno
\alpha_{i,3} - \alpha_{i,2}
&>& \alpha_{i,4} - \alpha_{i,3},
\ee
then individual $i$ makes more progress between time $2$ and $3$ than between time $3$ and $4$.

Under the proposed model with log odds
\beno
\eta_{i,j,t}
&=&
\log \dfrac{\mu_{i,j,t}}{1-\mu_{i,j,t}}
&=& \begin{cases}
\alpha_i + \beta_j - \gamma\, d(\bm{a}_{i,2}, \mT)
& \mbox{if $t=2$}
\\
\alpha_i + \beta_j - \gamma\, d(\bm{a}_{i,3}, \mT)
& \mbox{if $t=3$}
\\
\alpha_i + \beta_j - \gamma\, d(\bm{a}_{i,4}, \mT)
& \mbox{if $t=4$,}
\end{cases}
\ee
one can assess whether individual $i$ makes more progress between time $2$ and $3$ than between time $3$ and $4$ along the same lines,
by inspecting changes in log odds:
\beno
\eta_{i,j,3} - \eta_{i,j,2}
&=& \gamma\, d(\bm{a}_{i,3}, \mT) - \gamma\, d(\bm{a}_{i,2}, \mT)\s
\\
\eta_{i,j,4} - \eta_{i,j,3}
&=& \gamma\, d(\bm{a}_{i,4}, \mT) - \gamma\, d(\bm{a}_{i,3}, \mT).
\ee
Suppose that
\beno
\gamma\, d(\bm{a}_{i,3}, \mT) - \gamma\, d(\bm{a}_{i,2}, \mT)
&>& \gamma\, d(\bm{a}_{i,4}, \mT) - \gamma\, d(\bm{a}_{i,3}, \mT),
\ee
which,
upon dividing both sides by $\gamma$,
is equivalent to
\beno
d(\bm{a}_{i,3}, \mT) - d(\bm{a}_{i,2}, \mT)
&>& d(\bm{a}_{i,4}, \mT) - d(\bm{a}_{i,3}, \mT),
\ee
provided that $\gamma > 0$.
Then individual $i$ makes more progress between time 2 and 3 than between time 3 and 4,
because the log odds increase more during the first period than the second one.

In other words,
one can assess whether individual $i$ makes more progress during some periods than others by inspecting changes in log odds,
both under \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model and under the proposed model.
Under \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model,
inspecting changes in log odds amounts to inspecting changes of abilities $\alpha_{i,t}$.
By contrast,
under the proposed model,
inspecting changes in log odds amounts to inspecting changes of distances towards target $\mT$.
Both approaches to assessing progress are legitimate.
That being said,
the proposed model captures interactions between individuals and variables and provides a multidimensional interaction map,
whereas \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model cannot capture interactions between individuals and variables and provides a one-dimensional ability map.
We provide a detailed comparison with \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model in Section \ref{sec:comparison}.


==> figure/expected.scores.tex <==
There are other possible approaches to measuring progress:
e.g.,
one can base the assessment of progress on expected scores.

To demonstrate,
recall that the proposed statistical framework builds on generalized linear models.
In other words,
the responses $Y_{i,j,t}$ have statistical exponential-family distributions with canonical parameters $\eta_{i,j,t}$ \citep{Br86,Su19,efron22}.
In the language of statistical exponential families,
the proposed statistical framework measures progress based on the canonical parameterization of statistical exponential families.
An alternative would be to measure progress based on the mean-value parameterization of statistical exponential families,
that is,
based on expected scores.

To compare these alternative approaches to assessing progress,
let $\bm{Y}_i \coloneqq (Y_{i,j,t})_{1 \leq j \leq p,\, 1 \leq t \leq T}$\, be the vector of responses $Y_{i,j,t}$ of individual $i$ and let the distributions $\mbP_{\btheta,\bm{a}_{i,t},\bm{b}_j}$ of responses $Y_{i,j,t}$ be one-parameter exponential-family distributions (e.g., $Y_{i,j,t} \mid \mu_{i,j,t}$ $\ind$ $\mbox{Bernoulli}(\mu_{i,j,t})$ with mean $\mu_{i,j,t} \in (0, 1)$,\,
$Y_{i,j,t} \mid \mu_{i,j,t}\; \ind\; \mbox{Poisson}(\mu_{i,j,t})$ with mean $\mu_{i,j,t} \in (0, +\infty)$,\,
or $Y_{i,j,t} \mid \mu_{i,j,t},\, \sigma_{i,j,t}^2\; \ind\; N(\mu_{i,j,t},\, \sigma_{i,j,t}^2)$ with mean $\mu_{i,j,t} \in \mR$ and known variance $\sigma_{i,j,t}^2 \in (0, +\infty)$).
Then the probability density function of an exponential-family probability measure $\mbP_{\btheta,\bm{a}_{i,t},\bm{b}_j}$ dominated by a $\sigma$-finite measure $\nu$ can be represented as
\beno
f(y_{i,j,t} \mid \eta_{i,j,t})
&=& a_{i,j,t}(y_{i,j,t})\,  \exp(\eta_{i,j,t}\, s_{i,j,k}(y_{i,j,t}) - \psi_{i,j,t}(\eta_{i,j,t})),
\ee
where $a_{i,j,t}(y_{i,j,t}) \in [0, +\infty)$ is a function of $y_{i,j,t}$,\,
$\eta_{i,j,t} \equiv \eta_{i,j,t}(\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \bm{b}_j)) \in \mR$ is a canonical parameter,
$s_{i,j,t}(y_{i,j,t}) \in \mR$ is a sufficient statistic,
and
\beno
\psi_{i,j,t}(\eta_{i,j,t})
&\coloneqq& \dint_{\mY_{i,j,t}} \exp(\eta_{i,j,t}\, s_{i,j,k}(y_{i,j,t})) \dd \nu(y_{i,j,t})
\ee
ensures that $f(y_{i,j,t} \mid \eta_{i,j,t})$ integrates to $1$;
note that the general formulation above covers both the discrete setting (in which case $\nu$ may be counting measure) and the continuous setting (in which case $\nu$ may be Lebesgue measure).
As a result,
the probability density function of the response vector $\bm{Y}_i$ of individual $i$ can be represented as
\beno
f(\bm{y}_i \mid \bm\eta_i)
&=& \dprod_{j=1}^p\, \dprod_{t=1}^T f(y_{i,j,t} \mid \eta_{i,j,t})
&=& a_i(\bm{y}_i)\, \exp\left(\langle\bm\eta_i, s_i(\bm{y}_i)\rangle - \psi_i(\bta_i)\right),
\ee
where $a_i(\bm{y}_i) \coloneqq \prod_{j=1}^p \prod_{t=1}^T a_{i,j,t}(y_{i,j,t})$,\,
$\psi_i(\bta_i) \coloneqq \sum_{j=1}^p \sum_{t=1}^T \psi_{i,j,t}(\eta_{i,j,t})$,\,
and $\langle\bm\eta_i, s_i(\bm{y}_i)\rangle$ denotes the inner product of the vector of canonical parameters $\bm\eta_i \coloneqq (\eta_{i,j,t})_{1 \leq j \leq p,\, 1 \leq t \leq T}$ and the vector of sufficient statistics $s_i(\bm{y}_i) \coloneqq (s_{i,j,t}(y_{i,j,t}))_{1 \leq j \leq p,\, 1 \leq t \leq T}$.
In other words,
if the responses $Y_{i,j,t}$ have exponential-family distributions,
so does the response vector $\bm{Y}_i$ of individual $i$.
The parameter vector
\beno
\bm\mu_i(\bm\eta_i)
&\coloneqq& \mbE_{\bm\eta_i}\, s_i(\bm{Y}_i)
\ee
with coordinates $\mu_{i,j,t}(\bm\eta_i) \coloneqq \mbE_{\bm\eta_i}\, s_{i,j,t}(Y_{i,j,t})$ is known as the mean-value parameter vector of the exponential family.
Since the map $\bm\eta_i \mapsto \bm\mu_i(\bm\eta_i)$ is a homeomorphism and is therefore one-to-one \citep[][Theorem 3.6, p.\ 74]{Br86},
one can specify models and assess progress based on one of two parameterizations:
\bi
\item[1.] One can specify models and assess progress by specifying the canonical parameter vector $\bta_i$.\vspace{.1cm}
\item[2.] One can specify models and assess progress by specifying the mean-value parameter vector $\bmu_i(\bta_i) \coloneqq \mbE_{\bta_i}\, \bY_i$,
that is,
the expected score vector.
\ei
As a consequence,
one can measure progress based on either the canonical parameterization or the mean-value parameterization:
e.g.,
if the responses $Y_{i,j,t}$ of individual $i$ to variables $j$ have been recorded at $T = 2$ time points,
one could measure progress based on differences in mean-value parameters $\mu_{i,j,2}(\bm\eta_i)$ and $\mu_{i,j,1}(\bm\eta_i)$,
summed over all variables $j$:
\beno
\mbox{progress of individual $i$}
&\coloneqq& \dsum_{j=1}^p \left[\mu_{i,j,2}(\bm\eta_i) - \mu_{i,j,1}(\bm\eta_i)\right].
\ee
That being said,
it is common practice to specify generalized linear models by specifying the canonical parameters $\eta_{i,j,t}$ rather than the mean-value parameters $\mu_{i,j,t}(\bm\eta_i)$,
because the canonical parameterization helps incorporate covariates,
as explained in Section \ref{sec:other.approaches}.
That said,
both approaches to specifying generalized linear models are legitimate,
although we follow here the canonical route,
as do \citet{Rasch60}, 
\citet{jeon:21}, 
\citet{andersen:85},
and others.


==> figure/id.tex <==
\input{id.alpha.beta.tex}

In the special case $\mathbb{M} \coloneqq \mR^2$ and $d(\bm{a}_{i,t}, \mT) \coloneqq |\!|\bm{a}_{i,t} - \mT|\!|_2$,
the latent process model has the same identifiability issues as other Euclidean latent space models \citep[e.g.,][]{Hoff:2002},
in that the distances $d(\bm{a}_{i,t}, \mT)$ are invariant to reflection,
translation,
and rotation of the positions $\bm{a}_{i,t}$ of individuals $i$ at time $t$ and target $\mT$.
Such identifiability issues can be addressed by Procrustes matching \citep{Hoff:2002}.

\input{identifiability.issues.tex}


==> figure/interaction.tex <==
Note that the interactions between students $i$ and items $j$ are time-invariant,
because there is no good reason to believe that the positions $\bm{b}_j$ of items $j$ change during a short period of time and therefore the positions $\bm{b}_j$ of items $j$ are assumed to be time-invariant.


==> figure/interpret.alpha.tex <==
The terms $\alpha_i$,
$\beta_j$,
$\gamma$,
and $\gamma\, d(\bm{a}_{i,t}, \mT)$ can be interpreted as follows:
\bi
\item {\bf Weight $\alpha_i$.} 
The weight $\alpha_i$ quantifies the potential (ability) of individual $i$.
The potential (ability) $\alpha_i$ takes on values in $\mR$ and can therefore be as large as desired.
The potential (ability) $\alpha_i$ will be estimated from the observed responses $Y_{i,j,t}$ along with the weights $\beta_j$ and $\gamma$ and the distances $d(\bm{a}_{i,t}, \mT)$,
using the Bayesian approach in Section \ref{sec:inference}.\vspace{.1cm}
\item {\bf Weight $\beta_j$.}
The weight $\beta_j$ indicates how agreeable variable $j$ is:
The higher $\beta_j$ is,
the higher is the linear predictor $\eta_{i,j,t}$ and hence the mean response $\mu_{i,j,t}$,
holding everything else constant.\vspace{.1cm}
\item {\bf Weight $\gamma$.}
If $\gamma > 0$,
the distance term $\gamma\, d(\bm{a}_{i,t}, \mT)$ quantifies how far individual $i$ is below her potential (ability) $\alpha_i$.
For example,
if $d(\bm{a}_{i,t}, \mT) = 0$,
then individual $i$ has reached her potential (ability) $\alpha_i$ and cannot improve with respect to target $\mT$.
By contrast,
if $d(\bm{a}_{i,t}, \mT) > 0$,
then individual $i$ is below her potential (ability) $\alpha_i$ and can improve with respect to target $\mT$.\vspace{.1cm}
\item {\bf Making progress by reducing distance $d(\bm{a}_{i,t}, \mT)$.} 
The fact that the weights $\alpha_i$ and $\beta_j$ do not depend on time $t$ implies that the distance term $\gamma \, d(\bm{a}_{i,t}, \mT)$ captures the progress of individual $i$ towards target $\mT$.
Thus,
the more individual $i$ reduces the distance $d(\bm{a}_{i,t}, \mT)$ to target $\mT$,
the more progress $i$ makes,
assuming that $\gamma > 0$.
A mathematical description of the rate of progress as a function of the distance of individual $i$ to target $\mT$ is provided by Equations \eqref{d.reduction} and \eqref{rate.progress} in Section \ref{special.cases}.
\ei


==> figure/literature.tex <==
We provide a short comparison of the proposed latent process model with the \citet{Rasch60} and \citet{jeon:21} models of cross-sectional educational assessment data and \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model of longitudinal educational assessment data in Section \ref{sec:data.model}.
In addition, 
we provide a detailed comparison with \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model in Section \ref{sec:comparison}.


==> figure/mean.tex <==
It is worth noting that the definition $\mT \coloneqq (1/p) \sum_{j=1}^p \bm{b}_j$ of target $\mT$ as a function of the positions $\bm{b}_j$ of variables $j$ is motivated by the fact that the variables measure progress towards target $\mT$.
Therefore,
it hence makes sense to specify $\mT$ as a function of the variable positions $\bm{b}_j$.
The specification of target $\mT$ as the mean $(1/p) \sum_{j=1}^p \bm{b}_j$ of the variable positions $\bm{b}_j$ is simple and convenient,
although other specifications are possible.


==> figure/model.tex <==
Let
\beno
\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \bm{b}_j)
&\coloneqq& \mbE_{\btheta,\,\bm{a}_{i,t},\, \bm{b}_j}\; Y_{i,j,t}
\ee
be the mean response of individual $i$ to variable $j$ at time $t$ and $\eta_{i,j,t}$ be a link function,
which links the mean response $\mu_{i,j,t}$ to a linear predictor:
\beno 
\eta_{i,j,t}(\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \bm{b}_j))
&\coloneqq&
\begin{cases} 
\alpha_i + \beta_j - \gamma\; d(\bm{a}_{i,t}, \bm{b}_j)
& \mbox{if } t = 1\s
\\
\alpha_i + \beta_j - \gamma\; d(\bm{a}_{i,t}, \mT) 
& \mbox{if } t = 2, \dots, T,
\end{cases}
\ee
where $\mT \coloneqq (1/p) \sum_{j=1}^p \bm{b}_j$ is the target of interest,
measured by variables $j$ with positions $\bm{b}_j$,
and $\btheta \in \bTheta$ is the vector of weights $\alpha_i \in \mR$ ($i = 1, \dots, n$),\,
$\beta_j \in \mR$ ($j = 1, \dots, p$),\,
and $\gamma \in [0, +\infty)$.
\alert{
\input{interpret.alpha.tex}
\input{mean.tex}
} 

\alert{The data model can be viewed as an extension of the \citet{Rasch60} and \citet{jeon:21} models to longitudinal data.
The \citet{Rasch60} and \citet{jeon:21} models consider binary responses $Y_{i,j} \in \{0, 1\}$ observed at $T = 1$ time point and assume that $Y_{i,j} \mid \mu_{i,j}\, \ind\, \mbox{Bernoulli}(\mu_{i,j})$,
where $\logit(\mu_{i,j}) \coloneqq \alpha_i + \beta_j$ \citep{Rasch60} and $\logit(\mu_{i,j}) \coloneqq \alpha_i + \beta_j - \gamma\, d(\bm{a}_i, \bm{b}_j)$ \citep{jeon:21}.
\input{model.advantages.tex}
It is worth noting that the latent space should not be interpreted as an ability map,
because the potential (ability) of student $i$ is captured by $\alpha_i$.
Instead,
the latent space should be interpreted as an interaction map,
capturing interactions between students $i$ and items $j$:
e.g.,
a large distance $d(\bm{a}_{i,1}, \bm{b}_j)$ between student $i$ and item $j$ at time $1$ indicates that the mean response $\mu_{i,j,1}$ of student $i$ to item $j$ is lower than would be expected based on the potential (ability) $\alpha_i$ of student $i$ and the easiness $\beta_j$ of item $j$.
\input{interaction.tex}
}

\alert{In addition to inheriting the advantages of the \citet{jeon:21} model,
the proposed model helps assess
\bi
\item whether student $i$ makes progress towards learning target $\mT$,
based on changes of the distance $d(\bm{a}_{i,t}, \mT)$ as a function of time $t$;
\item how much progress student $i$ makes towards learning target $\mT$,
based on changes of the distance $d(\bm{a}_{i,t}, \mT)$,
and how much uncertainty is associated with such assessments;
\item whether student $i$ makes more progress during some periods than others;
\item how much more progress student $i$ can make in the future.
\ei
\input{diff.logit.tex}
}


==> figure/other.approaches.tex <==
There are other possible approaches to measuring progress:
e.g.,
one can base the assessment of progress on expected scores.

To demonstrate,
recall that the proposed statistical framework builds on generalized linear models.
In other words,
the responses $Y_{i,j,t}$ have statistical exponential-family distributions with canonical parameters $\eta_{i,j,t}$ \citep{Br86,Su19,efron22}.
It can be shown that the statistical exponential-family distributions of the responses $Y_{i,j,t}$ imply that the vectors of responses $\bm{Y}_i \coloneqq (Y_{i,j,t})_{1 \leq j \leq p,\, 1 \leq t \leq T}$ likewise have statistical exponential-family distributions canonical parameter vector $\bta_i$ with coordinates $\eta_{i,j,t}$ and the mean-value parameter vector $\bmu_i(\bta_i) \coloneqq \mbE_{\bta_i}\, \bY_i$ with coordinates $\mu_{i,j,t}(\bta_i) \coloneqq \mbE_{\bta_i}\, Y_{i,j,t}$:
mathematical details can be found in Supplement \ref{sec:expected.scores}. 
In statistical exponential families,
it is well-known that the map $\bta_i \mapsto \bmu_i(\bta_i)$ is one-to-one:
see,
e.g., 
Theorem 3.6 on page 74 of \citet{Br86}.
The one-to-one relationship of $\bta_i$ and $\bmu_i(\bta_i) \coloneqq \mbE_{\bta_i}\, \bY_i$ implies that one can specify models and assess progress based on one of two parameterizations:
\bi
\item[1.] One can specify models and assess progress by specifying the canonical parameter vector $\bta_i$.\vspace{.1cm}
\item[2.] One can specify models and assess progress by specifying the mean-value parameter vector $\bmu_i(\bta_i) \coloneqq \mbE_{\bta_i}\, \bY_i$,
that is,
the expected score vector.
\ei
Due to the one-to-one relationship of $\bta_i$ and $\bmu_i(\bta_i)$,
one can go back and forth between $\bta_i$ and $\bmu_i(\bta_i)$,
regardless of how one specifies the model \citep[although the map $\bta_i \mapsto \bmu_i(\bta_i)$ may be nonlinear and may not be available in closed form: see, e.g.,][]{ScSt19}.
In practice,
it is common to specify generalized linear models by specifying the canonical parameters $\eta_{i,j,t}$ rather than the mean-value parameters $\mu_{i,j,t}(\bta_i)$,
because the canonical parameterization allows to incorporate covariates.

To demonstrate that the canonical parameterization allows to incorporate covariates,
consider binary responses $Y_{i,j,t} \mid \mu_{i,j,t}\, \ind\, \mbox{Bernoulli}(\mu_{i,j,t})$ along with a time-dependent covariate $x_{i,t} \in \mR$, 
e.g., 
the income of the parents of student $i$ at time $t$.
To specify models of binary responses $Y_{i,j,t} \mid \mu_{i,j,t}\, \ind\, \mbox{Bernoulli}(\mu_{i,j,t})$ with time-dependent covariates $x_{i,t} \in \mR$,
it is common practice to leverage the canonical parameterization $\bta_i$ of generalized linear models,
that is,
the logit link:
\beno
\eta_{i,j,t}
&=& \log\dfrac{\mu_{i,j,t}}{1-\mu_{i,j,t}}
&=&
\begin{cases}
\alpha_i + \beta_j - \gamma\; d(\bm{a}_{i,t}, \bm{b}_j) + \delta\, x_{i,t}
& \mbox{if } t = 1\s
\\
\alpha_i + \beta_j - \gamma\; d(\bm{a}_{i,t}, \mT) + \delta\, x_{i,t}
& \mbox{if } t = 2, \dots, T,
\end{cases}
\ee
where $\delta \in \mR$ is the weight of covariate $x_{i,t} \in \mR$.
By contrast,
it is less convenient to specify models of binary responses $Y_{i,j,t} \mid \mu_{i,j,t}\, \ind\, \mbox{Bernoulli}(\mu_{i,j,t})$ with time-dependent covariates $x_{i,t} \in \mR$ by using the mean-value parameterization $\bmu_i(\bta_i)$:
e.g.,
a linear model of the form 
\beno
\mu_{i,j,t}(\bta_i) 
&\coloneqq& \mbE_{\bta_i}\, Y_{i,j,t} 
&=& \alpha_i + \beta_j - \gamma\; d(\bm{a}_{i,t}, \bm{b}_j) + \delta\, x_{i,t}
\ee
would not be appropriate,
not least because the mean response $\mu_{i,j,t}$ could be less than $0$ or greater than $1$---despite the fact that the response $Y_{i,j,t}$ is either $0$ or $1$.

In addition to having advantages for specifying models and estimating models \citep[see advantages 1--5 in Section 1 of][pp.~628--629]{ScKrBu17},
the canonical parameterization facilitates the assessment of progress compared with the mean-value parametrization,
that is,
the expected scores:
e.g.,
suppose one assesses the progress of individual $i$ based on the changes in the expected score of individual $i$ between time $1$ and $2$:
\beno
\mbox{progress of individual $i$}
&\coloneqq& \dsum_{j=1}^p \left[\mu_{i,j,2}(\bm\eta_i) - \mu_{i,j,1}(\bm\eta_i)\right].
\ee
Then changes of the expected score could be due to 
\bi
\item changes in time-dependent covariates $x_{i,t} \in \mR$,
e.g.,
changes in the income of the parents of student $i$ between time $1$ and $2$;
\item the progress $\lambda_{i,2}$ of individual $i$ between time $1$ and $2$;
\item a combination of changes in time-dependent covariates $x_{i,t} \in \mR$ and the progress of individual $i$ between time $1$ and $2$.
\ei
Using expected scores,
it is not straightforward to assess whether changes of expected scores are due to changes in time-dependent covariates or changes in the progress of individual $i$ or both.

While both approaches (based on the canonical and mean-value parameterization, that is, expected scores) to specifying models and assessing progress are legitimate,
we follow the canonical route,
as do \citet{andersen:85} and others: see \citet{Su19} and \citet{efron22}.
It is worth repeating that the simulations in Section \ref{sec:interaction} and the applications in Sections \ref{sec:depression} and \ref{sec:math} demonstrate the advantages of the interaction map provided by the latent process model over the one-dimensional ability map provided by \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model,
and that the latent process model enables a novel look at mental health and online educational assessments in disadvantaged subpopulations.
A more technical discussion can be found in Supplement \ref{sec:expected.scores}.


==> id.alpha.beta.tex <==
We discuss identifiability issues along with possible solutions,
following a Bayesian approach.
A Bayesian approach to addressing identifiability issues deviates from a non-Bayesian approach,
because the posterior density is proportional to the likelihood times the prior density.
As a result,
identifiability issues can be addressed through the prior.

A well-known issue of the classic \citet{Rasch60} model and its extensions---including the proposed latent process model---is that the weights $\alpha_i$ and $\beta_j$ cannot be all estimated,
unless additional restrictions are imposed.
We follow convention by imposing the constraints $\mu_\alpha \coloneqq 0$ and $\mu_\beta \coloneqq 0$:
see,
e.g.,
page 316 of \citet{GeHi07}.
Such constraints are widely used for addressing the identifiability issues of the \citet{Rasch60} model and other item response models in a Bayesian setting:
see,
e.g.,
\citet{Al92} and \citet{Cu10}.


==> identifiability.issues.tex <==
An additional identifiability issue arises from the fact that,
for all $c \in (0, 1) \cup (1, +\infty)$,
\beno
\eta_{i,j,t}(\mu_{i,j,t}(\btheta,\,  \bm{a}_{i,t},\, \bm{b}_j))
&\coloneqq& \alpha_i + \beta_j - \gamma\, |\!|\bm{a}_{i,t} - \mT|\!|_2
&=& \alpha_i + \beta_j - \dfrac{\gamma}{c}\, |\!|c\, \bm{a}_{i,t} - c\, \mT|\!|_2,
\ee
where $\mT \coloneqq (1/p) \sum_{j=1}^p \bm{b}_j$.
Such identifiability issues can be addressed by constraining either the positions $\bm{a}_{i,t}$ of individuals $i$ at time $t$ or the positions $\bm{b}_j$ of variables $j$ (but not both).
We constrain the positions $\bm{b}_j$ of variables $j$,
adapting the constraint of \citet{HaRaTa07}:
\beno
\sqrt{\dfrac{1}{p} \dsum_{j=1}^p |\!|\bm{b}_j|\!|_2^2}
&=& 1.
\ee
We do not constrain the positions $\bm{a}_{i,t}$ of individuals $i$ at time $t$.


==> interaction.tex <==
Note that the interactions between students $i$ and items $j$ are time-invariant,
because there is no good reason to believe that the positions $\bm{b}_j$ of items $j$ change during a short period of time and therefore the positions $\bm{b}_j$ of items $j$ are assumed to be time-invariant.


==> model.advantages.tex <==
The proposed model can be viewed as an extension of these models to binary and non-binary responses $Y_{i,j,t}$ observed at $T \geq 2$ time points $t \in \{1, \dots, T\}$,
and reduces to
\bi
\item the \citet{Rasch60} model when binary responses $Y_{i,j} \in \{0, 1\}$ are observed at $T = 1$ time point,
the link function is the logit link,
and $\gamma = 0$;\vspace{.1cm}
\item the \citet{jeon:21} model when binary responses $Y_{i,j} \in \{0, 1\}$ are observed at $T = 1$ time point,
the link function is the logit link,
and $\gamma \in [0, +\infty)$.
\ei
\input{monotone.tex}


==> model.short.tex <==
Let
\beno
\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \bm{b}_j)
&\coloneqq& \mbE_{\btheta,\,\bm{a}_{i,t},\, \bm{b}_j}\; Y_{i,j,t}
\ee
be the mean response of individual $i$ to variable $j$ at time $t$ and $\eta_{i,j,t}$ be a link function,
which links the mean response $\mu_{i,j,t}$ to a linear predictor:
\beno 
\eta_{i,j,t}(\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \bm{b}_j))
&\coloneqq&
\begin{cases} 
\alpha_i + \beta_j - \gamma\; d(\bm{a}_{i,t}, \bm{b}_j)
& \mbox{if } t = 1\s
\\
\alpha_i + \beta_j - \gamma\; d(\bm{a}_{i,t}, \mT) 
& \mbox{if } t = 2, \dots, T,
\end{cases}
\ee
where $\mT \coloneqq (1/p) \sum_{j=1}^p \bm{b}_j$ is the target of interest,
measured by variables $j$ with positions $\bm{b}_j$,
and $\btheta \in \bTheta$ is the vector of weights $\alpha_i \in \mR$ ($i = 1, \dots, n$),\,
$\beta_j \in \mR$ ($j = 1, \dots, p$),\,
and $\gamma \in [0, +\infty)$.
\alert{\input{interpret.alpha.tex}} 
\alert{The fact that the weights $\alpha_i$ and $\beta_j$ do not depend on time $t$ implies that the distance term $d(\bm{a}_{i,t}, \mT)$ captures the progress of individual $i$ towards target $\mT$.
}
\alert{\input{mean.tex}} 


==> old/conclusion.tex <==
\section{Future directions}

We have introduced a latent process model that helps monitor progress towards hard-to-measure targets.
There are multiple interesting directions of future research.
For example,
in some applications there are multiple targets of interest, 
all of them related,
and it is of interest to monitor progress towards all of them.
A specific example is the learning progress of students with respect to algebra and geometry,
which are two distinct but related targets.
It would be possible to build a latent process model that helps monitor progress with respect to both algebra and geometry by embedding both of them into a low-dimensional Euclidean space.
A related problem consists of monitoring learning progress with respect to two distinct and related problems with a known,
hierarchical relationship:
e.g.,
to learn the method of maximum likelihood,
students first need to learn the notion of probability density functions.
Latent process models tackling these and other problems constitute interesting directions of future research,
enabling educators to monitor learning progress through visual maps.


==> old/discussion.metric.space.tex <==
An open issue is how to select the geometry of the metric space $(\mathbb{M}, d)$.
In the statistical analysis of {\em network data,}
recent work by \citet{LuChMc23} introduced a promising approach to selecting the geometry of latent space models of network data,
although the approach of \citet{LuChMc23} falls outside of the Bayesian framework considered here.
In the statistical analysis of {\em educational data,}
we are not aware of comparable work.
Having said that,
we expect that the pioneering work of \citet{LuChMc23} paves the way for Bayesian approaches to selecting the geometry of the underlying space,
for models of network data as well as for models of educational data.
In the special case $\mathbb{M} \coloneqq \mR^q$ ($q \geq 1$) and $d(\bm{a}_{i,t}, \mT) \coloneqq |\!|\bm{a}_{i,t} - \mT|\!|_2$,
an additional issue may arise,
in that the dimension $q$ of $\mR^q$ may not be known.
Since we are interested in dimension reduction (embedding both individuals and variables in a low-dimensional space) and helping professionals without a strong statistics background assess the progress of individuals towards  a target $\mT$ of interest,
it is tempting to choose $\mathbb{M} \coloneqq \mR^q$ ($q \geq 1$) and $d(\bm{a}_{i,t}, \mT) \coloneqq |\!|\bm{a}_{i,t} - \mT|\!|_2$ along with $q = 2$ or $q = 3$,
although hyperbolic spaces and other metric spaces would be interesting alternatives.


==> old/general.tex <==
In its most general form,
the process model makes two assumptions about the set $\mathbb{M}$.
First,
the set $\mathbb{M}$ is equipped with a distance function $d$,
so that the distances between the individuals $i$,
the variables $j$, 
and the target $\mT$ can be quantified.
Second,
the set $\mathbb{M}$ is convex,
so that the positions $\bm{a}_{i,t} \coloneqq (1-\lambda_{i,t})\; \bm{a}_{i,t-1} + \lambda_{i,t}\; \mT$ of individuals $i$ at time $t$ are contained in the set $\mathbb{M}$,
provided that $\bm{a}_{i,t-1} \in \mathbb{M}$ and $\mT \in \mathbb{M}$.
The process model does not require additional assumptions about the set $\mathbb{M}$.


==> old/identifiability.issues.tex <==
An additional issue is that,
for all $c \in (0, 1) \cup (1, +\infty)$,
\beno
\eta_{i,j,t}(\mu_{i,j,t}(\btheta,\,  \bm{a}_{i,t},\, \bm{b}_j))
&\coloneqq& \alpha_{i,t} + \beta_{j,t} - \gamma\, |\!|\bm{a}_{i,t} - \mT|\!|_2
&=& \alpha_{i,t} + \beta_{j,t} - \dfrac{\gamma}{c}\, |\!|c\, \bm{a}_{i,t} - c\, \mT|\!|_2,
\ee
where $\mT \coloneqq (1/p) \sum_{j=1}^p \bm{b}_j$.
Such identifiability issues can be addressed by constraining either the positions $\bm{a}_{i,t}$ of individuals $i$ at time $t$ or the positions $\bm{b}_j$ of variables $j$ (but not both).
We constrain the positions $\bm{b}_j$ of variables $j$,
adapting the constraint of \citet{HaRaTa07}:
\beno
\sqrt{\dfrac{1}{p} \dsum_{j=1}^p |\!|\bm{b}_j|\!|_2^2}
&=& 1.
\ee
We do not constrain the positions $\bm{a}_{i,t}$ of individuals $i$ at time $t$.


==> old/latent.space.tex <==
To monitor the progress of individuals towards a target of interest $\mT$,
we assume that the individuals and the variables measuring progress towards target $\mT$ have positions in a shared metric space $(\mathbb{M},\, d)$, 
consisting of a set $\mathbb{M}$ and a distance function $d: \mathbb{M}^2 \mapsto [0, +\infty)$.
We assume that the set $\mathbb{M}$ is a convex set and allow the metric space $(\mathbb{M},\, d)$ to be Euclidean or non-Euclidean.
In statistical network analysis \citep{HuKrSc12,SmAsCa19},
two broad classes of latent space models can be distinguished,
based on the geometry of the underlying metric space:
Euclidean latent space models \citep{HpRaHm01} and latent models with intrinsic hierarchical structure,
based on ultrametric space \citep{ScSn03} or hyperbolic space \citep{hyperbolic}.
The proposed probabilistic framework can accommodate these and other metric spaces.
Having chosen a metric space $(\mathbb{M},\, d)$,
based on ease of visualization or statistical model selection methods \citep[e.g.,][]{LuChMc23},
we assume that individuals $i$ have positions $\bm{a}_{i,t} \in \mathbb{M}$ at time $t$ and move towards the target of interest $\mT \in \mathbb{M}$,
measured by variables $j$ with positions $\bm{b}_{j} \in \mathbb{M}$.
The position of the target $\mT$ is assumed to be time-invariant. 
It is possible to extend the proposed latent process model to time-varying targets,
provided that data warrant the resulting increase in model complexity,
but we do not consider such extensions here.


==> old/mcmc_old.tex <==

\section{Markov chain Monte Carlo algorithm}
\label{appendix:mcmc}

We approximate the posterior by combining the following Markov chain Monte Carlo steps by cycling or mixing \citep*{Tl94}:

\begin{enumerate}
  
    \item Sample $\beta_{j,t}$ from its full conditional distribution: 
    \[ 
\beta_{j,t} \sim \mbox{N}\left(m_\beta, {v_\beta^2} \right),
   \]
  \begin{align*}
         m_\beta & =   \left(\frac{1}{\sigma^2_\beta} + \sum_i \, \omega_{i,j,t} \right)^{-1} \, \left( \sum_i \, K_{i,j,t} - \sum_i \, \omega_{i,j,t} \, \gamma \, g(\bm{a}_{i,t}, \mT)  \right) \\
         {v_\beta^2} &=  \left(\frac{1}{\sigma^2_\beta} + \sum_i \, \omega_{i,j,t} \right)^{-1}, 
  \end{align*} 
  where $K_{i,j,t} = Y_{i,j,t} - {1}/{2}$, and ${K_{i,j,t}}/{\omega_{i,j,t}} \sim \mbox{N}(0,1)$ with $\omega_{i,j,t} \sim \mbox{PG} \left(1, \beta_{j,t} + \gamma \,  g(\bm{a}_{i,t}, \mT) \right)$ and $\mbox{PG} (b,c)$ is a P\'{o}lya-Gamma distribution with $b > 0$ and $c \in \mathbb{R}$ \citep{polson:13}.

% \textcolor{red}{Michale: don't want to use $*$ for posterior means and variances? alternatives? 
% Plus, I realize that we use $\beta_{j}$ -- this is a bit complicated here; the formula for mean and variance above are slightly different when $beta_j$ are the same  at both time points and when  $beta_j$ are different  
% }


    \item Sample $\alpha{i,t}$ from its full conditional distribution: 
    \[ 
\alpha_{j,t} \sim \mbox{N}\left(m_\alpha, {v_\alpha^2} \right),
   \]
  \begin{align*}
         m_\alpha & =   \left(\frac{1}{\sigma^2_\alpha} + \sum_i \, \omega_{i,j,t} \right)^{-1} \, \left( \sum_i \, K_{i,j,t} - \sum_i \, \omega_{i,j,t} \, \gamma \, g(\bm{a}_{i,t}, \mT)  \right) \\
         {v_\alpha^2} &=  \left(\frac{1}{\sigma^2_\alpha} + \sum_i \, \omega_{i,j,t} \right)^{-1}, 
  \end{align*} 

    \item Sample $\sigma_{\alpha}^2$ from the Inverse Gamma distribution 
    \[
    \sigma_{\alpha}^2 \sim \mbox{Inv-Gamma}\left(a_{\sigma_{\alpha}} + \frac{N}{2}, b_{\sigma_{\alpha}} + \frac{\sum_i \alpha_i^2}{2}\right),
    \]   


    \item Sample $\gamma$ from its full conditional distribution: 
    \[ 
\gamma \sim \mbox{Half-Normal}\left(m_\gamma, v^2_\gamma \right),
   \]
 {\small 
  \begin{align*}
         m_\gamma & = \left(\frac{1}{\sigma^2_\gamma} +  \sum_i \sum_j \sum_t \, \omega_{i,t,} \, g(\bm{a}_{i,t}, \mT)^2 \right)^{-1}\, \left ( \sum_i \sum_j \sum_t \,K_{i,j,t} \, g(\bm{a}_{i,t}, \mT)  - \sum_i \sum_j \sum_t \, \omega_{i,j,t} \, \beta_{j,t} \, g(\bm{a}_{i,t}, \mT) \right)  \\
         {v_\gamma^2} &=  \left(\frac{1}{\sigma^2_\gamma} +  \sum_i \sum_j \sum_t \, \omega_{i,t,} \, g(\bm{a}_{i,t}, \mT)^2 \right)^{-1}. 
  \end{align*} 
  }
     \item Propose $\lambda_{i,t}^\star$ from a symmetric proposal distribution and accept the proposal with probability
    \[
\min\left(1,\; \frac{f\Big(\lambda_{i,t}^\star \mid \bm{K},\, \bm{\omega},\,  \bm{A},\, \bm{B},\, \bm{\beta},\,  \gamma \Big)} {f\Big(\lambda_{i,t}^{(l)} \mid \bm{K},\, \bm{\omega},\, \bm{A},\, \bm{B},\, \bm{\beta},\, \gamma \Big)}\right).
\]

    \item Propose $\bm{a}_{i,1}^\star$ from a symmetric proposal distribution and accept the proposal with probability
\[
    \min \left(  1,\; {\frac{f\Big(\bm{a}_i^\star \mid \bm{K},\, \bm{\omega},\,  \bm{A}_{-i},\, \bm{B},\, \bm{\beta},\, \la, \, \gamma  \Big)} {f \Big( \bm{a}_i^{(l)} \mid \bm{K},\, \bm{\omega},\,  \bm{A}_{-j},\, \bm{B},\, \bm{\beta},\, \la, \,\gamma \Big) } }  \right) ,
\]


where $\bm{A}_{-i} = (\bm{a}_1, \dots, \bm{a}_{i-1}, \bm{a}_{i+1}, \dots, \bm{a}_n)$.





    \item Propose $\bm{b}_j^\star$ from a symmetric proposal distribution and accept the proposal with probability
    \[
\min\left(1,\; \frac{f\Big(\bm{b}_j^\star \mid \bm{K},\, \bm{\omega},\,  \bm{A},\, \bm{B}_{-j},\, \bm{\beta},\, \la,\, \gamma  \Big)} 
    {f\Big(\bm{b}_j^{(l)} \mid \bm{K},\, \bm{\omega},\,  \bm{A},\, \bm{B}_{-j},\, \bm{\beta},\, \la,\, \gamma  \Big)} \right)   ,
    \]
    where $\bm{B}_{-j} = (\bm{b}_1, \dots, \bm{b}_{j-1}, \bm{b}_{j+1}, \dots, \bm{b}_q)$.

\hide{     

\item Sample $\mT$ from its full conditional distribution: 
    \[
  \mT \sim \mbox{MVN}_q\left(\bm{m}_{\mT},\; {v_{\mT}^2} \, \bm{I}_q \right)
\]
  \begin{align*}
         \bm{m}_{\mT} & = \left(n  + \frac{1} {{\sigma_{{\mT}}}^2}\right)^{-1} \, \left( \sum_{j=1}^p \, \bm{b}_j \right)\s 
         \\
         {v_{\mT}^2} &= \left(\frac{1} {{\sigma_{{\mT}}}^2} + n \right)^{-1}. 
  \end{align*} 

}

\item Sample $\pi_{i,t}$ from its full conditional distribution: 
\[
\pi_{i,t} \sim \mbox{Beta} \left(a_\pi + r_{i,t}, \, b_\pi + (1- r_{i,t}) \right),
\]
where $\pi_{i,t} \coloneqq \mbP(r_{i,t} = 1 \mid \pi_{i,t})$ and $r_{i,t} \in \{0,1 \}$ is sampled from its full conditional distribution:
% \[
% r_{i,t} \sim \mbox{Bernoulli} 
% \left( \frac{1} { 1 + \frac{ (1- \pi_{i,t})}{\pi_{i,t}}  
% \frac{\left(2\pi \sigma_0^2 \right)^{-\frac{1}{2}} \mbox{exp} \left( -\frac{1}{2\sigma_0^2}  \left(\lambda_{i,t} - \mu_0 \right)^2 \right)   }  
% {\left(2\pi \sigma_1^2 \right)^{-\frac{1}{2}} \mbox{exp} \left( -\frac{1}{2\sigma_1^2}  \left(\lambda_{i,t} - \mu_1 \right)^2 \right)   } }    
% \right)
% \]
\[
r_{i,t} \sim \mbox{Bernoulli} 
\left( \left( 1 + \frac{ (1- \pi_{i,t})}{\pi_{i,t}}  
\frac{\left(2\pi \sigma_0^2 \right)^{-\frac{1}{2}} \exp \left( -\frac{1}{2\sigma_0^2}  \left(\logit(\lambda_{i,t}) - \mu_0 \right)^2 \right)   }  
{\left(2\pi \sigma_1^2 \right)^{-\frac{1}{2}} \exp \left( -\frac{1}{2\sigma_1^2}  \left(\logit(\lambda_{i,t}) - \mu_1 \right)^2 \right)   } \right)^{-1}  
\right).
\]
\end{enumerate}

As proposal distributions,
we use multivariate Gaussians centered at the current values of the quantities in question,
with diagonal variance-covariance matrices.
The variances are set to achieve acceptance rates between .3 and .4. 

\hide{

To address the identifiability issues reviewed in Section 2.4 of the manuscript,
we constrain the standard deviation of 
$Z \coloneqq 
(\bm{a}_{1,1}^\prime, \dots, \bm{a}_{1,T}^\prime, \dots, \bm{a}_{n,1}^\prime, \dots, \bm{a}_{n,T}^\prime,\, \bm{b}_{1}^\prime, \dots, \bm{b}_{p}^\prime)$ to be $1$.

}

==> old/model.tex <==
Let
\beno
\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \bm{b}_j)
&\coloneqq& \mbE_{\btheta,\,\bm{a}_{i,t},\, \bm{b}_j}\; Y_{i,j,t}
\ee
be the mean response of individual $i$ to variable $j$ at time $t$ and $\eta_{i,j,t}$ be a link function,
which links the mean response $\mu_{i,j,t}$ to a linear predictor:
\beno
\eta_{i,j,t}(\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \bm{b}_j))
&\coloneqq&
\begin{cases}
\alpha_{i,t} + \beta_{j,t} - \gamma\; d(\bm{a}_{i,t}, \bm{b}_j)
& \mbox{if } t = 1\s
\\
\alpha_{i,t} + \beta_{j,t} - \gamma\; d(\bm{a}_{i,t}, \mT)
& \mbox{if } t = 2, \dots, T,
\end{cases}
\ee
where $\mT \coloneqq (1/p) \sum_{j=1}^p \bm{b}_j$ is the target of interest,
measured by variables $j$ with positions $\bm{b}_j$,
and $\btheta \in \bTheta$ is a vector of parameters with coordinates $\alpha_{i,t} \in \mR$,\,
$\beta_{j,t} \in \mR$,\,
and $\gamma \in \mR$.
The data model can be viewed as an extension of the classic model of \citet{Rasch60} and the more recent model of \citet{jeon:21} from cross-sectional data to longitudinal data.
The \citet{Rasch60} and \citet{jeon:21} models consider binary responses $Y_{i,j} \in \{0, 1\}$ observed at a single time point and assume that $Y_{i,j} \mid \mu_{i,j}\, \ind\, \mbox{Bernoulli}(\mu_{i,j})$,
where $\logit(\mu_{i,j}) = \alpha_i + \beta_j$ \citep{Rasch60} and $\logit(\mu_{i,j}) = \alpha_i + \beta_j - \gamma\; d(\bm{a}_i, \bm{b}_j)$ \citep{jeon:21}.
The above model can be viewed as an extension of the \citet{Rasch60} and \citet{jeon:21} models to binary responses observed at two or more time points $t \in \{2, \dots, T\}$,
and reduces to
\bi
\item the \citet{Rasch60} model when $T = 1$ and $\gamma = 0$;\s
\item the \citet{jeon:21} model when $T = 1$. 
\ei



==> old/other.approaches.tex <==
\subsection{Other approaches to measuring progress}
\label{sec:other.approaches}

There are other possible approaches to measuring progress,
both within and outside of the proposed statistical framework.

To demonstrate, 
recall that the proposed statistical framework builds on generalized linear models.
In other words,
the responses $Y_{i,j,t}$ have exponential-family distributions $\mbP_{\btheta,\bm{a}_{i,t},\bm{b}_j}$ \citep{Su19,efron22}.
In the language of exponential families,
the proposed statistical framework measures progress based on the canonical parameterization of the exponential family.
An alternative would be to measure progress based on the mean-value parameterization of the exponential family.

To explain,
let $\bm{Y}_i = (Y_{i,j,t})_{1 \leq j \leq p,\, 1 \leq t \leq T}$\, be the vector of responses $Y_{i,j,t}$ of individual $i$.
The exponential-family distributions $\mbP_{\btheta,\bm{a}_{i,t},\bm{b}_j}$ of responses $Y_{i,j,t}$ are one-parameter exponential families (e.g., $Y_{i,j,t} \sim \mbox{Bernoulli}(\mu_{i,j,t})$ with mean $\mu_{i,j,t} \in (0, 1)$, 
$Y_{i,j,t} \sim \mbox{Poisson}(\mu_{i,j,t})$ with mean $\mu_{i,j,t} \in (0, +\infty)$,
or $Y_{i,j,t} \sim N(\mu_{i,j,t},\, \sigma_{i,j,t}^2)$ with mean $\mu_{i,j,t} \in \mR$ and known $\sigma_{i,j,t}^2 \in (0, +\infty)$).
Then the probability density function of $\mbP_{\btheta,\bm{a}_{i,t},\bm{b}_j}$ with respect to a dominating $\sigma$-finite measure $\nu$ can be represented as
\beno
f(y_{i,j,t} \mid \eta_{i,j,t})
&=& a_{i,j,t}(y_{i,j,t})\,  \exp(\eta_{i,j,t}\, s_{i,j,k}(y_{i,j,t}) - \psi_{i,j,t}(\eta_{i,j,t})),
\ee
where $a_{i,j,t}(y_{i,j,t}) \in [0, +\infty)$ is a function of $y_{i,j,t}$,\,
$\eta_{i,j,t} \equiv \eta_{i,j,t}(\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \bm{b}_j)) \in \mR$ is a canonical parameter,
$s_{i,j,t}(y_{i,j,t}) \in \mR$ is a sufficient statistic,
and
\beno
\psi_{i,j,t}(\eta_{i,j,t})
&=& \dint \exp(\eta_{i,j,t}\, s_{i,j,k}(y_{i,j,t})) \dd \nu(y_{i,j,t})
\ee
ensures that $f(y_{i,j,t} \mid \eta_{i,j,t})$ integrates to $1$;
note that the general formulation above covers both the discrete setting (in which case $\nu$ may be counting measure) and the continuous setting (in which case $\nu$ may be Lebesgue measure).
% and that $\int g \dd \nu$ denotes the Lebesgue integral of a measurable function $g$.
As a result,
the probability density function of the response vector $\bm{Y}_i$ of individual $i$ can be represented as
\beno
f(\bm{y}_i \mid \bm\eta_i)
&=& \dprod_{j=1}^p\, \dprod_{t=1}^T f(y_{i,j,t} \mid \eta_{i,j,t})
&=& a_i(\bm{y}_i)\, \exp\left(\langle\bm\eta_i, s_i(\bm{y}_i)\rangle - \psi_i(\bta_i)\right),
\ee
where $a_i(\bm{y}_i) = \prod_{j=1}^p \prod_{t=1}^T a_{i,j,t}(y_{i,j,t})$ and $\psi_i(\bta_i) = \sum_{j=1}^p \sum_{t=1}^T \psi_{i,j,t}(\eta_{i,j,t})$.
Here, 
$\langle\bm\eta_i, s_i(\bm{y}_i)\rangle$ denotes the Euclidean inner product of the vector of canonical parameters $\bm\eta_i = (\eta_{i,j,t})$ and the vector of sufficient statistics $s_i(\bm{y}_i) = (s_{i,j,t}(y_{i,j,t}))$.
In other words,
if the responses $Y_{i,j,t}$ have exponential-family distributions,
so does the response vector $\bm{Y}_i$ of individual $i$.

The parameter vector 
\beno
\bm\mu_i(\bm\eta_i) 
&\coloneqq& \mbE_{\bm\eta_i}\, s_i(\bm{Y}_i)
\ee
with coordinates $\mu_{i,j,t}(\bm\eta_i) \coloneqq \mbE_{\bm\eta_i}\, s_{i,j,t}(\bm{Y}_i)$ is known as the mean-value parameter vector of the exponential family.
Since the mean-value parameter map in exponential families is one-to-one \citep[][Theorem 3.6, p.\ 74]{Br86},
one can parameterize the model by using either the canonical parameter vector $\bm\eta_i$ or the mean-value parameter vector $\bm\mu_i(\bm\eta_i)$.
As a consequence,
one can measure progress based on the canonical parameterization $\bm\eta_i$ or the mean-value parameterization $\bm\mu_i(\bm\eta_i)$:
e.g.,
if the responses $Y_{i,j,t}$ of individual $i$ to variables $j$ have been recorded at $T = 2$ time points,
one could measure progress based on differences in mean-value parameters $\mu_{i,j,2}(\bm\eta_i)$ and $\mu_{i,j,1}(\bm\eta_i)$,
summed over the responses of individual $i$ to variables $j$:
\beno
\dsum_{j=1}^p \left[\mu_{i,j,2}(\bm\eta_i) - \mu_{i,j,1}(\bm\eta_i)\right].
\ee
That being said,
the mean-value parameterization is less convenient for the purpose of model selection,
e.g.,
the problem of determining whether students make progress.
As pointed out above,
the ability to determine whether individuals make progress towards the target of interest is an advantage of the proposed statistical approach.
In general,
it is common practice to base model selection of generalized linear models on the canonical parameterization rather than the mean-value parameterization of exponential families.
Therefore,
by assessing whether individuals make progress based on the canonical parameterization rather than the mean-value parameterization,
we follow convention.


==> old/paper3_conclusion.tex <==
\section{Discussion}
\label{sec:discussion}

We have introduced a latent process model for monitoring progress towards a hard-to-measure target of interest,
with a number of possible extensions.

As an example,
it may be of interest to monitor the progress of individuals towards two or more related targets:
e.g.,
to understand the Bayesian notion of posterior probability,
students first need to understand the notion of probability.
Thus,
there is a sequence of two related learning targets (learning the notion of probability and learning the notion of posterior probability),
and it may be of interest to monitor the progress of students towards both of them.
The latent process model can be extended to deal with such scenarios.
A second example is regress,
the opposite of progress.
Capturing regress is of interest in applications to mental health problems,
because the mental health of patients may deteriorate rather than improve.
Extensions of latent process models tackling these and other challenges constitute interesting directions for future research.


==> old/part1.tex <==
\section{Introduction}
\label{sec:intro}

The recent shift to remote learning and work has aggravated long-standing problems,
such as the problem of monitoring the mental health of individuals \citep[e.g.,][]{daly:20, holmes:20} and the progress of students towards learning targets \citep[e.g.,][]{engzell:21, kuhfeld:20, bansak:20}.

We introduce a novel approach to monitoring the progress of individuals towards a hard-to-measure target of interest.
Examples are measuring the progress of individuals with mental health problems or the progress of students towards learning targets.
Both examples have in common that there is a target of interest (e.g., improving mental health or the understanding of learning concepts) and measuring progress towards the target is more challenging than measuring changes in physical quantities (e.g., temperature) or medical conditions (e.g., cholesterol levels),
but a set of variables is available for measuring progress towards the target. 
If, 
e.g., 
the goal is to monitor the progress of students towards learning targets,
measurements can be collected by paper-and-pencil or computer-assisted educational assessments,
whereas progress in terms of mental health can be monitored by collecting data on well-being by using surveys along with physical measurements related to stress by using wearable devices.

We propose a latent process model with a view to monitoring the progress of individuals towards a target of interest,
measured by a set of variables. 
The latent process model is based on the idea of embedding both individuals and the target in a shared metric space.
The fact that individuals are embedded in the same metric space as the target makes it possible to assess how much progress individuals make towards the target,
and helps quantify how much more progress individuals can make towards the target in the future.
We first provide a motivating example in Section \ref{example},
then review existing models in Section \ref{sec:literature},
and point out in Section \ref{sec:comparison} that special cases of the latent process model can be viewed as a geometric version of existing models.

\subsection{Motivating example}
\label{example}

We consider data collected on the online learning platform My Math Academy \citep{bang:22}.
The data consist of responses $Y_{i,j,t} \in \{0, 1\}$ provided by 421 kindergarten children, first- and second-grade students $i \in \{1, \dots, 421\}$ to 30 problems $j \in \{1, \dots, 30\}$ at two time points $t \in \{1, 2\}$.
The problems measure progress with respect to the understanding of numbers and arithmetic operations.
A more detailed description of the data can be found in Section \ref{sec:math}.
In practice,
educators,
students, 
parents,
and other stakeholders may wish to assess how much progress students made between the first and second time point and how much more progress the students can make in the future,
in addition to quantifying the uncertainty about these assessments.
\hide{
We first estimate a conventional logit model from the My Math Academy data \citep{andersen:85},
assuming $Y_{i,j,t} \mid \mu_{i,j,t}\, \ind\, \mbox{Bernoulli}(\mu_{i,j,t})$ ($\mu_{i,j,t} \in (0, 1)$) with $\logit(\mu_{i,j,t}) = \beta_j + \vartheta_{i,t}$ ($\beta_j \in \mR$, $\vartheta_{i,t} \in \mR$).
To demonstrate the advantages of the proposed latent process model over the logit model,
we select Hispanic students $A$,
$B$,
$C$,
and $D$.
The logit model was estimated by marginal maximum likelihood methods using {\tt R} package {\tt lme4} \citep{lme4:09}.
The empirical Bayes estimates and standard errors of $\vartheta_{i,t}$ in Table \ref{tab:growth_random_mm} demonstrate:
\bi
\item The logit model helps assess progress of students towards the target of interest (task A): 
e.g.,
the estimates $\widehat\vartheta_{B,1} = .502$ and $\widehat\vartheta_{B,2} = 2.106$ suggest that student $B$ made substantial progress towards the target of interest,
and the uncertainty about the estimates $\widehat\vartheta_{B,1}$ and $\widehat\vartheta_{B,2}$ can be quantified by the standard errrors $.375$ and $.222$,
respectively. 
\vspace{.1cm}
\item The logit model is less useful for quantifying how much more progress students can make towards the target of interest in the future:
e.g.,
to quantify how much more progress student $B$ could make at a third assessment in the future,
one could make a prediction based on the estimated expectations $\mbE_{\widehat\vartheta_{B,1}, \widehat\vartheta_{B,2}, \widehat\beta_1, \dots, \widehat\beta_{30}}\, Y_{B,j,t}$ for $j \in \{1, \dots, 30\}$ and $t \in \{1, 2\}$,
but there are 60 of them and it is unclear how to combine those 60 estimates. 
% $\widehat\vartheta_{B,2} = 2.106$ and,
%since $\vartheta_{B,2}$ could be much larger than $2$ (e.g., $\vartheta_{B,3}$ could be 4 or 5A naive approach to quantifying how much more progress students can make in the future would be to inspect student $B$ with estimated parameter $\widehat\vartheta_{B,2} = 2.106$ at time $2$ has room for improvement,
%because $\vartheta_{B,2} \in (-\infty,\, +\infty)$ can be much larger than $2.106$.
\ei
\begin{table}[ht]
\begin{tabular}{ccrrrccc}
    Student $i$ && $\widehat\vartheta_{i,1}$ (time 1) && $\widehat\vartheta_{i,2}$ (time 2) & Correct (time 1) & Correct (time 2)\\ 
  \hline
$A$ && -.789 (.364) && .039 (.167) & 33.3\% & 60.0\% \\ 
$B$ && .502 (.375) && 2.106 (.222) & 56.7\% & 96.7\% \\ 
$C$ && -.344 (.361) && 1.635 (.197) & 36.7\% & 93.3\% \\ 
$D$ && -1.642 (.396) && -.140 (.181) & 13.3\% & 60.0\% \\ 
   \hline
\end{tabular}
\caption{\label{tab:growth_random_mm}
Empirical Bayes estimates $\widehat\vartheta_{i,t}$ and standard errors of the parameters $\vartheta_{i,t}$ of the $\logit(\mu_{i,j,t}) = \beta_j + \vartheta_{i,t}$\, model based on responses by Hispanic students $i \in \{A, B, C, D\}$ to problems $j \in \{1, \dots, 30\}$ at times $t \in \{1, 2\}$,
collected on the online learning platform My Math Academy.
The columns ``Correct" show the percentages of correct responses at times $t \in \{1, 2\}$.}
\end{table}

That said,
the room for improvement suggested by the logit model turns out to be a mirage.
}

% \noindent\begin{minipage}{\textwidth}

% \s\s\s\s

\begin{figure}[t]
\begin{center}
\begin{tikzpicture}
[scale=.65, 
  transform shape, node distance=2cm,
  roundnode/.style={circle, draw=black, thick, minimum size=10mm},
  squarednode/.style={rectangle, draw=black, thick, minimum size=6mm},
  arrow/.style = {semithick,-Stealth},
  dotnode/.style={fill,inner sep=0pt,minimum size=2pt,circle} 
]

% x axis 
\draw   (-7,0) -- (8, 0) ;
% y axis 
\draw   (0,-4.5) -- (0,5) ;

% Target:
\draw [fill=green!10,draw=none] (6.33 ,3.51) circle (2cm) node [scale=1.5]  {$\mT$} ; % 

% Original position of student C:
\draw [fill] (-2.46 , 1.89) circle (1mm)  ;
\draw (-2.86,  1.89) node [scale=1.5] {$C$}; 

% person C (G) t2 
\draw [fill] (2.08, 2.74) circle (1mm)  ;
\draw[->, thick,dashed] (-2.46,  1.89)  -- (1.98, 2.74); 

% person A (E) t1
\draw [fill] (-2.49, -0.60) circle (1mm)  ;
\draw (-2.89, -0.60) node [scale=1.5] {$A$} ;

% person A (E) t2 
\draw [fill] (0.00, 0.57) circle (1mm)  ;
\draw[->, thick,dashed] (-2.49 ,-0.60)   -- (-0.2, 0.57)  ; 


% person D (H) t1
\draw [fill] (-4.29, -2.70) circle (1mm)  ;
\draw (-4.69 ,-2.70) node [scale=1.5] {$D$} ; 

% person D (H) t2 
\draw [fill] (-0.03 ,-0.21) circle (1mm)  ;
\draw[->, thick,dashed] (-4.29 ,-2.70)  -- (-0.23, -0.21)   ; 


% person B (F) t1
\draw [fill] (0.12 ,-1.29) circle (1mm)  ;
\draw (-0.32 ,-1.29) node [scale=1.5] {$B$} ; 

% person B (F) t2 
\draw [fill] (5.25, 2.67) circle (1mm)  ;
\draw[->, thick,dashed] (0.12, -1.29)  -- (5.05, 2.67) ; 

\end{tikzpicture}
\end{center}
\caption{An embedding of Hispanic students $A$, $B$, $C$, and $D$ along with learning target $\mT$,
the understanding of numbers and arithmetic operations,
into $\mR^2$.
These results are based on a Bayesian approach to the proposed latent process model,
using data collected on the online learning platform My Math Academy.
The posterior medians of the positions of students $A$, $B$, $C$, and $D$ at the first and second test are represented by circles and connected by arrows.
The results reveal that some students made more progress than others,
and that student $B$ may be close to reaching the target while students $A$, $C$, and $D$ may need additional assistance.
Note that the distances between the students and the target $\mT$ affect the responses of students,
but the distances between the students do not affect the responses.
\label{examplefigure}}
\end{figure}

\s\s\s

We demonstrate that the proposed latent process model can help inform such assessments.
The latent process model is described in Section \ref{sec:probabilistic.framework}.
To demonstrate the model,
we use a Bayesian approach to estimating the model from the My Math Academy data,
embedding the students along with the target of interest into $\mR^2$.
The target is concerned with the understanding of numbers and arithmetic operations.
Figure \ref{examplefigure} shows the learning progression map of four Hispanic students $A$, $B$, $C$, and $D$ and suggests that student $B$ may be close to reaching the target,
while students $A$, $C$, and $D$ may need additional assistance.
Having said that,
there is uncertainty about the rate of progress of student $B$,
which measures how much the distance between student $B$ and the target is reduced between time $1$ and $2$ and is quantified by a real number between $0$ (no progress) and $1$ (target reached):
While the posterior median of $B$'s rate of progress is $.832$,
the 95\% posterior credible interval $[.337,\, .997]$ indicates that the posterior distribution is long-tailed and there is non-negligible uncertainty about $B$'s rate of progress.
We review these results in more detail in Section \ref{sec:math}.
% The data support these conclusions:
% Student $B$ provided correct responses to 96.7\% of the problems in the second test.
% Thus,
% the data confirm that student $B$ is close to reaching the learning target,
% although the data do not provide a measure of uncertainty about how much progress student $B$ made,
% and how much more progress student $B$ can make in the future.
\hide{
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrrr}
  \hline
 & grade & gender & race & free lunch & median & low.ci & high.ci & pi \\ 
  \hline
A & 0.000 & 1.000 & 1.000 & 0.000 & 0.318 & 0.107 & 0.526 & 0.719 \\ 
B & 1.000 & 1.000 & 1.000 & 1.000 & 0.832 & 0.337 & 0.997 & 0.985 \\ 
C & 1.000 & 0.000 & 1.000 & 1.000 & 0.527 & 0.260 & 0.816 & 0.948 \\ 
D & 1.000 & 0.000 & 1.000 & 1.000 & 0.411 & 0.201 & 0.615 & 0.882 \\ 
   \hline
\end{tabular}
\end{table}
}

The motivating example described above demonstrates that the latent process model 
\bi
\item provides a visual representation of how much progress students made;
\item provides a visual representation of how much more progress students can make in the future;
\item helps quantify the uncertainty about these assessments based on the posterior distribution;
\item facilitates the dissemination of such assessments among educators, students, parents, and other stakeholders, 
by providing a visual map of individual progress and quantifying the rate of progress by a real number between $0$ (no progress) and $1$ (target reached).
% rather than differences in abilities (which can be arbitrarily large).
\ei
In short,
these advantages enable non-statisticians to assess progress towards hard-to-measure targets,
without requiring a deep understanding of statistical models.
We are developing a Shiny app to facilitate the dissemination of the proposed latent process model among practitioners.

\subsection{Existing models}
\label{sec:literature}

Many existing models of longitudinal, educational data are based on the classic model of \citet{andersen:85}.
\citeauthor{andersen:85} assumed that responses $Y_{i,j,t} \in \{0, 1\}$ of individuals $i$ to problems $j$ at time $t$ are independent $\mbox{Bernoulli}(\mu_{i,j,t})$ ($\mu_{i,j,t} \in (0, 1)$) random variables,
where
\beno\logit(\mu_{i,j,t}) 
&=& \beta_j + \vartheta_{i,t},
\ee
where $\beta_j \in \mR$ and $\vartheta_{i,t} \in \mR$ can be interpreted as the easiness of problem $j$ and the ability of individual $i$ at time $t$, 
respectively. 
% , with  $(\vartheta_{i,1}, \dots, \vartheta_{i,T}) \ind MVN(\mathbf{0}, \bSigma)$ ($\bSigma \succ 0$).  
% For example, suppose we have $Y_{i,j,t} \in \mathcal{Y}_{i,j,t}$ be the binary response of respondent $i$  ($i = 1, \dots, n$) to item $j$  ($j = 1, \dots, p$) from a test at time $t$ ($t = 1, \dots, T$).  
% %and $Y_{i,j,t} \in \{0, 1\}$. 
% For simplicity, the test measures a single target (knowledge, attitude, or skill set), and the same test (with the identical set of items) was given at different measurement points. Assuming that item parameters are invariant across time points, \cite{andersen:85} presented a multidimensional model for longitudinal item response data: 
% \begin{equation}
% \label{eq:0}
% \begin{array}{llllll}
% \mbox{logit} (\mathbb{P} (Y_{i,j,t} = 1 \mid \alpha_{i,t}, \, \beta_j ) \;:=\; 
% \alpha_{i,t} + \beta_j,
% & t = 1, \dots, T.
% \end{array}
% \end{equation}
%\noindent where $\alpha_{i,t} \in \mR$ is the latent trait level of respondent $i$ at time $t$,
%and  $\beta_j \in \mR$ is the overall easiness of item $i$. 
%The vector of occasion-specific latent traits $\boldsymbol{\vartheta}_i = (\vartheta_{i,1}, \dots, \vartheta_{i,T})' \sim N(\mathbf{0}, \Sigma)$.  
Using \citeauthor{andersen:85}'s model,
the progress of individual $i$ between time $1$ and $2$ can be assessed based on the difference $\vartheta_{i,2} - \vartheta_{i,1}$.
\citet{embretson:91} reparameterized \citeauthor{andersen:85}'s model by modeling changes in abilities via $\vartheta_{i,t}^\star \coloneqq \vartheta_{i,t} - \vartheta_{i,t-1}$.
% (for $t >1$) in addition to the latent initial state $\vartheta_{i,1}$.   
%extended in several other ways, for example, to measure multiple for multidimensional tests by considering additional latent traits tapped into the associated attributes (or learning targets) \citep[e.g.,][]{wang:20}. 
%Two limitations of these approaches are: (1) the number of latent variables increases as the number of occasions and/or the number of learning targets or attributes increase, and (2) the change is not modeled as a smooth function of time. To resolve this issue, 
\citeauthor{andersen:85}'s model has been extended by,
e.g., 
capturing temporal dependence when the same variables are used to measure progress over time \citep[e.g.,][]{cai:10} and addressing multiple learning topics at each time point \citep[e.g.,][]{wang:20, huang:15}.  
Other approaches model changes in abilities as a function of time \cite[e.g.,][]{pastor:06, wilson:12}
% :
% e.g.,
% one can specify a linear growth model as 
% $\alpha_{i,t}$:  
%linear or polynomial models to reduce the number of latent variables and measure a smooth latent change. 
%For example, \cite{pastor:06} specified a linear growth model for $\alpha_{i,t}$
% $\vartheta_{i,t} = \delta_{1,i} + \delta_{2,i}\, \text{time}_{i,t} + \epsilon_{i,t}$ ($\delta_{1,i} \in \mR$,\, $\delta_{2,i} \in \mR$,\, $\epsilon_{i,t} \in \mR$).
%, \,\,\, \epsilon_{i,t} \ind N(0,\sigma_\epsilon^2)
%$
% where $\delta_{1,i} \in \mR$ and $\delta_{2,i} \in \mR$.
% are the random intercept and random slope, representing person $i$'s initial status and growth rate, respectively, with 
%$(\delta_{1,i}, \delta_{2,i})' \sim N(\mathbf{0}, \Sigma)$. % and  The time-specific random effects $\epsilon_{i,t}$ are assumed to follow a normal distribution, $\epsilon_{i,t} \sim N(0,\sigma_\epsilon^2)$. 
%Linear growth models have been extended by,
%e.g.,
and incorporate first-order autoregressive structure \citep{jeon:2016,segawa:05}.
A limitation of these models is that more than two time points are required to estimate them. 
% model with random intercepts and slopes.  
% \textcolor{red}{[mj: we don't have to say that $\delta_{1,i}$ and $\delta_{2,i}$ are random intercepts and slopes? and there is a correlation between them. ]}

In conclusion, 
\citeauthor{andersen:85}'s model and its extensions help assess the progress of individuals based on differences in abilities.
That said,
these models have shortcomings:
e.g.,
the fact that the progress of individuals is assessed based on differences in abilities and these differences can be arbitrarily large
% By contrast,
% the proposed latent process model quantifies the rate of progress by a real number between $0$ (no progress) and $1$ (target reached).
%\textcolor{red}{[mj: it may be useful to clarify why arbitrarily large difference ability scores are problematic? Also, I think an identical value can have different relative standings in different samples. For example, a difference score of 2 may be small in one sample but large in another sample. ]} 
%Thus, it may be difficult to interpret how large or small one's latent change is; and an identical number may have a different relative standing in different samples.  % can only be discussed in the sample and relative to other people or other time points. 
%In other words, one's latent change cannot be evaluated in an absolute sense; 
makes it challenging to assess how much more progress individuals can make in the future.
%\textcolor{red}{[mj: I wonder whether we can stress this somehow. I don't believe any approaches with continuous scores offer this kind of information. For discrete latent variable models (with e.g., mastery and non-mastery), it is much simpler. if a student shows a transition of no mastery to no mastery for an attribute, then he still needs to master the attribute. }]
By contrast,
the proposed latent process facilitates the assessment of how much more progress individuals can make in the future,
because the rate of change of each individual is bounded below by $0$ (no progress) and bounded above by $1$ (target reached).
For example,
if the 95\% posterior credible interval of an individual's rate of change is $[.80, .99]$,
one can conclude that the individual is,
with high posterior probability,
close to reaching the target.
% because the rate of change is bounded above by $1$ (target reached).

\subsection{Outline}

We introduce the proposed latent process model in Section \ref{sec:probabilistic.framework} and outline a Bayesian approach to statistical inference in Section \ref{sec:inference}.
Simulation results and applications to the My Math Academy and CourseKata data can be found in Sections \ref{sec:simulations}, 
\ref{sec:math}, 
and \ref{sec:coursekata},
respectively.

\section{Latent process model}
\label{sec:probabilistic.framework}

Consider responses $Y_{i,j,t} \in \mathcal{Y}_{i,j,t}$ by individuals $i \in \{1, \dots, n\}$ ($n \geq 1$) to variables $j \in \{1, \dots, p\}$ ($p \geq 1$) at times $t \in \{1, \dots, T\}$ ($T \geq 2$).
To leverage data from multiple sources (e.g., self-reported mental health assessments collected by surveys and physical measurements related to stress collected by wearable devices),
we allow responses $Y_{i,j,t}$ to be binary ($\mathcal{Y}_{i,j,t} = \{0, 1\}$),
count-valued ($\mathcal{Y}_{i,j,t} = \{0, 1, \dots\}$),
real-valued ($\mathcal{Y}_{i,j,t} = \mR$),
or a combination of them.

To monitor the progress of individuals towards a target of interest $\mT$,
we assume that the individuals and the target $\mT$ have positions in a shared metric space $(\mathbb{M},\, d)$, 
consisting of a space $\mathbb{M}$ and a distance function $d: \mathbb{M}^2 \mapsto [0, +\infty)$.
To facilitate visual representations,
we consider $\mathbb{M} \coloneqq \mR^q$ and $d(\bm{a}, \bm{b}) \coloneqq \sqrt{\sum_{k=1}^q (a_k - b_k)^2}$,
where $(\bm{a}, \bm{b}) \in \mathbb{M}^2$ and $q \geq 1$ is assumed known. 
In line with the literature on latent space models in statistical network analysis \citep[e.g.,][]{HpRaHm01},
it is natural to choose either $q = 2$ or $q = 3$,
to enable visualization in $\mR^2$ or $\mR^3$.
%It is worth noting that the distances between the students and the target $\mT$ affect the responses of students,
%but the distances between the students do not affect the responses.
%\textcolor{red}{[mj: Q1. $\mathbb{M}^2$ means a two-dimensional metric space? if so, can we say $\mathbb{M}^2$  but $q \geq 1 $ for $\mR^q$? perhaps I don't understand the notation $\mathbb{M}^2$. Q2. we say that dimension $q \geq 1 $ for $\mR^q$  is assumed to known to facilitate visualization, meaning $q=1,2, \text{or} 3$. In the end, we choose $q=2$ in all of our analyses. But from figure 2 and section 2.2., it is clear that we model "distances towards the target" for individuals, meaning that we essentially need only one dimensional space regardless of the choice of $q$. The JASA AE also pointed that out. I think it would be useful to be transparent about this. It might be okay to say that we will work with a 2-dimensional space because visualization in a two-dimensional space is more appealing than one-dimensional space (and we follow the convention of the network/latent space modeling literature). what do you think?]} 

We assume that individuals $i$ have positions $\bm{a}_{i,t} \in \mR^q$ at time $t$ and move towards the target of interest $\mT \in \mR^q$,
measured by variables $j$ with positions $\bm{b}_{j} \in \mR^q$.
The position of the target $\mT$ is assumed time-invariant.
It is possible to extend the proposed latent process model to time-varying targets,
provided that data warrant the resulting increase in model complexity,
but we do not consider such extensions here.

We assume that the responses $Y_{i,j,t} \in \mY_{i,j,t}$ are independent conditional on the positions $\bm{a}_{i,t}$ of individuals $i$ at time $t$ and target $\mT$,
and are distributed as
\beno
Y_{i,j,t} \mid \btheta,\, \bm{a}_{i,t},\, \mT 
&\ind& \mbP_{\btheta,\bm{a}_{i,t},\, \mT},
\ee
where $\mbP_{\btheta,\bm{a}_{i,t},\, \mT}$\, is a distribution with support $\mY_{i,j,t}$ and $\btheta \in \bTheta$ is a vector of parameters.

We divide the description of the probabilistic framework into 
\bi
\item the data model:
the model that generates the responses $Y_{i,j,t}$ conditional on the positions $\bm{a}_{i,t}$ of individuals $i$ at time $t$ and target $\mT$ (Section \ref{sec:data.model});
\item the process model:
the process that determines whether and how much individuals $i$ move towards target $\mT$ (Section \ref{sec:latent.process.model});
\item the priors of the model parameters (Section \ref{sec:prior}).
\ei
We review identifiability issues in Section \ref{sec:id} and explain in Section \ref{sec:comparison} that special cases of the latent process model can be viewed as a geometric version of existing models.

\subsection{Data model}
\label{sec:data.model}

The data model describes how the responses $Y_{i,j,t}$ are generated conditional on the positions $\bm{a}_{i,t}$ of individuals $i$ at time $t$ and the target of interest $\mT$. 

To leverage data from multiple sources (e.g., binary, count-, and real-valued responses),
we assume that the responses $Y_{i,j,t}$ are generated by generalized linear models \citep{Su19}.
Let
\beno
\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \mT) 
&\coloneqq& \mbE_{\btheta,\,\bm{a}_{i,t},\, \mT}\; Y_{i,j,t}
\ee
be the mean response of individual $i$ to variable $j$ at time $t$ and $\eta_{i,j,t}$ be a link function, 
which links the mean response $\mu_{i,j,t}$ to a linear predictor:
\beno
\eta_{i,j,t}(\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \mT)) 
&\coloneqq& \alpha_{i,t} + \beta_{j,t} + \gamma\; g(\bm{a}_{i,t},\, \mT),
\ee
where $\btheta \in \bTheta$ is a vector of parameters with coordinates $\alpha_{i,t} \in \mR$,\,
$\beta_{j,t} \in \mR$,\,
and $\gamma \in \mR$, 
and $g$ is a function of the positions $\bm{a}_{i,t}$ of individual $i$ at time $t$ and target $\mT$.
The data model can be viewed as an extension of the \citet{Rasch60} model to longitudinal data.
The \citeauthor{Rasch60} model considers binary responses $Y_{i,j} \in \{0, 1\}$ observed at a single time point and assumes $Y_{i,j} \mid \mu_{i,j}\, \ind\, \mbox{Bernoulli}(\mu_{i,j})$,
where $\logit(\mu_{i,j}) = \alpha_i + \beta_j$.
The data model extends the \citeauthor{Rasch60} model to binary responses observed at two or more time points $t$ and assumes $Y_{i,j,t} \mid \mu_{i,j,t}\, \ind\, \mbox{Bernoulli}(\mu_{i,j,t})$,
where $\logit(\mu_{i,j,t}) = \alpha_{i,t} + \beta_{j,t} + \gamma\; g(\bm{a}_{i,t},\, \mT)$. 
Covariates can be added in the data model or the process model, 
as discussed in Section \ref{sec:latent.process.model}.
It is worth noting that the data model assumes that the mean responses of individuals depend on the positions $\bm{a}_{i,t}$ of individuals $i$ at time $t$ and target $\mT$,
but do not depend on the distances between individuals.

\paragraph{Individual weights $\alpha_{i,t}$}

Motivated by identifiability issues,
we set $\alpha_{i,t} = 0$.
We review identifiability issues in Section \ref{sec:id}.

\paragraph{Variable weights $\beta_{j,t}$}

The weights $\beta_{j,t}$ of variables $j$ can depend on time $t$,
for two reasons.
First,
different variables may be used at different time points to measure progress towards target $\mT$.
Second,
even when the same variables are used,
the weights of variables may change over time
\citep[e.g.,][]{goldstein:83, wells:02}: 
e.g.,
a measure-theoretic problem may have been perceived as a simple problem in a Ph.D.\ qualifying exam in Statistics in the 1980s,
but the same problem may be perceived as a hard problem in the age of data science,
so the weight of the problem may have changed over time.

\paragraph{Function $g(\bm{a}_{i,t}, \mT)$ with weight $\gamma$}

The function $g(\bm{a}_{i,t}, \mT)$ with weight $\gamma$ determines how the positions $\bm{a}_{i,t}$ of individual $i$ at time $t$ and target $\mT$ affect the linear predictor $\eta_{i,j,t}$ and hence the mean response $\mu_{i,j,t}$. 
To facilitate interpretation,
we consider the specification $g(\bm{a}_{i,t}, \mT) \coloneqq \exp(- d(\bm{a}_{i,t}, \mT))$ with weight $\gamma > 0$.
The chosen specification deviates from the tradition in statistical network analysis \citep[e.g.,][]{Hoff:2002,ScSn03,HaRaTa07,sewell2015latent,SmAsCa19}.
In statistical network analysis,
one of the more common specifications are distance functions of the form $g(\bm{a}_i, \bm{a}_j) \coloneqq d(\bm{a}_i, \bm{a}_j)$ with weight $\gamma = -1$,
assuming that pairs of nodes $i$ and $j$ of a random network have time-invariant positions $\bm{a}_i$ and $\bm{a}_j$ in $\mR^q$.
While simple and convenient,
the interpretation of the negative distance function is less straightforward,
because the notion of progress has a positive rather than a negative annotation.
By contrast,
the distance function $g(\bm{a}_{i,t}, \mT) \coloneqq \exp(- d(\bm{a}_{i,t}, \mT))$ with weight $\gamma > 0$ increases the linear predictor by a real number between $0$ and $\gamma > 0$,
because $\gamma\, g(\bm{a}_{i,t}, \mT) = \gamma$ when $d(\bm{a}_{i,t}, \mT) = 0$ and $\gamma\, g(\bm{a}_{i,t}, \mT) \downarrow 0$ as $d(\bm{a}_{i,t}, \mT) \uparrow +\infty$. 
In other words,
the linear predictor is increased by a real number between $0$ and $\gamma$,
depending on how much the distance between the positions of individual $i$ and target $\mT$ is reduced between time $t-1$ and $t$.

\subsection{Process model}
\label{sec:latent.process.model}

\setcounter{figure}{1}

\begin{figure}[t]
\centering
\begin{tikzpicture}
[scale=1, 
  transform shape, node distance=2cm,
  roundnode/.style={circle, draw=black, thick, minimum size=10mm},
  squarednode/.style={rectangle, draw=black, thick, minimum size=6mm},
  arrow/.style = {semithick,-Stealth},
  dotnode/.style={fill,inner sep=0pt,minimum size=2pt,circle} % <- this is new
]

% x axis 
\draw   (0,0) -- (10, 0) ;
% y axis 
\draw   (0,0) -- (0,7) ;

% variable groups 
\draw [fill=green!10,draw=none] (3,5) circle (1.2cm) node [scale=1]  {$\mT$} ; 

% variables in group A 
\draw [fill] (2.9,5.7) circle (.6mm)  ;
\draw [fill] (2.6,4.5) circle (.6mm)  ;
\draw [fill] (3.5,4.9) circle (.6mm)  ;
\draw [fill] (3.7,5.8) circle (.6mm)  ;
\draw [fill] (2.1,5) circle (.6mm)  ;

% person 1 time 1 
\draw [fill] (2,1.3) circle (1mm)  ;
\draw (1.3,1.3) node [scale=1] {$\bm{a}_{i,1}$} ;

% shortest path to group A 
\draw[->,dashed] (2,1.3) -- (3,4.8) ; 

% person 1 time 2 
\draw [fill] (2.55,3.3) circle (1mm)  ;
\draw (1.8,3.3) node [scale=1] {$\bm{a}_{i,2}$} ;

% movement of person 1 
\draw[->, thick,dashed] (2,1.3) -- (2.55,3.2) ; 

% person 2 time 1 (disadvantaged)
\draw [fill] (7,1) circle (1mm)  ;
\draw (7.3,.6) node [scale=1] {$\bm{a}_{j,1}$} ;

% person 2 time 2 
\draw [fill] (6,1.9) circle (1mm)  ;
\draw (6.6,2.1) node [scale=1] {$\bm{a}_{j,2}$} ;

% movement of person 2
\draw[->, dashed] (7,1) -- (3,4.8); 
\draw[->, thick,dashed] (7,1) -- (6, 1.9); 

% j1 to A 
\draw (2,1.3) to [out=10,in =-20]  (2.55,3.3); 
\draw (3.5,2.3) node [scale=1]  {$\lambda_{i,2}$} ;

% j2 to A 
\draw (7,1) to [out=-120,in =-120]  (6, 1.9); 
\draw (5.8,.8) node [scale=1] {$\lambda_{j,2}$} ;

\end{tikzpicture}
\caption{Two individuals $i$ and $j$ make progress towards a target of interest $\mT \in \mR^2$,
measured by variables that are represented by points in the green-colored ball.
The rates of progress $\lambda_{i,2}$ and $\lambda_{j,2}$ determine how much the distance of $i$ and $j$ to target $\mT$ is reduced between time $1$ and $2$,
respectively. 
\label{fg:target}
}
\end{figure}

The process model determines whether and how much progress individuals make towards the target of interest $\mT$.

Consider an individual $i$ moving towards target $\mT$,
as demonstrated in Figure \ref{fg:target}.
We assume that the target $\mT$ and the variables measuring progress towards target $\mT$ are located at positions
\beno
\mT \mid \sigma_{\mT}^2 
&\sim& \mbox{MVN}_q(\bm{0}_q,\, \sigma_{\mT}^2\,\, \bm{I}_q),
&& \sigma_{\mT}^2\, >\, 0
\ee
and
\beno
\bm{b}_j \mid \mT,\, \sigma_b^2 
&\iid& \mbox{MVN}_q(\mT,\, \sigma_b^2\,\, \bm{I}_q),
&& \sigma_b^2\, >\, 0,
\ee
where $\mbox{MVN}_q$ denotes a $q$-variate Gaussian distribution,
$\bm{0}_q \in \mR^q$ is a $q$-dimensional null vector,
and $\bm{I}_q \in \mR^{q \times q}$ is an $q \times q$ identity matrix.
% and $\sigma_{\mT}^2$ and $\sigma_b^2$ are specified hyperparameters.

The process model assumes that the position $\bm{a}_{i,t}$ of individual $i$ at time $t$ is generated as follows.
First,
the position $\bm{a}_{i,1}$ of individual $i$ at time $t=1$ is generated by sampling 
\beno
\bm{a}_{i,1} \mid \sigma_a^2 
&\iid& \mbox{MVN}_q(\bm{0}_q,\, \sigma_a^2\,\, \bm{I}_q),
&& \sigma_a^2\, >\, 0.
\ee
% where $\sigma_a^2$ is a specified hyperparameter.
Second,
the position $\bm{a}_{i,t}$ of individual $i$ at time $t \in \{2, \dots, T\}$ is determined by
\be
\label{aposition}
\bm{a}_{i,t}
&\coloneqq& (1-\lambda_{i,t})\; \bm{a}_{i,t-1} + \lambda_{i,t}\; \mT,
&& t = 2, \dots, T,
\ee
where $\lambda_{i,t} \in [0, 1]$ can be interpreted as the rate of progress of individual $i$ towards target $\mT$ between time $t-1$ and $t$.
Thus,
if individual $i$ makes progress,
$i$ moves towards target $\mT$ on the shortest path between $\bm{a}_{i,t-1}$ and $\mT$.
The rate of progress $\lambda_{i,t}$ determines how much the distance between the positions of individual $i$ and target $\mT$ is reduced between time $t-1$ and $t$:
\beno
d(\bm{a}_{i,t},\, \mT)
&=& (1 - \lambda_{i,t})\; d(\bm{a}_{i,t-1},\, \mT),
&& t = 2, \dots, T.
\ee
A random term could be added to the right-hand side of \eqref{aposition} to allow individuals to deviate from the shortest path between $\bm{a}_{i,t-1}$ and $\mT$,
but we prefer to keep the process model as simple as possible,
because the moves of individuals in $\mR^q$ are unobserved.

If predictors $\bX_{i,t} \in \mR^w$ ($w \geq 1$) of the rate of progress $\lambda_{i,t}$ of individual $i$ between time $t-1$ and $t$ are available (e.g., demographic or educational background variables),
the predictors can be incorporated into the rate of progress as follows:
\be
\label{covariates}
\lambda_{i,t}(\bm\delta,\, \bX_{i,t})
&\coloneqq& \logit^{-1}\left(\delta_{0,t} + \dsum_{k=1}^w\, \delta_{k,t}\; x_{i,t,k}\right),
&& t = 2, \dots, T,
\ee
where $\delta_{0,t} \in \mR$ is an intercept and $\delta_{1,t}$, $\dots$, $\delta_{w,t} \in \mR$ are the weights of predictors $x_{i,t,k}$.
The intercept $\delta_{0,t}$ and the weights $\delta_{1,t}, \dots, \delta_{w,t}$  of covariates $x_{i,t,k}$ can depend on time $t$.

%\textcolor{red}{[mj: the JASA AE criticized that one could do this after we estimated lambda values for individuals. Do you want to comment on that point]}

\hide{

\subsubsection{Two or more targets}
\label{sec:two} 

If there are two or more targets but the targets are unrelated,
one can study progression towards those targets by constructing separate learning progression maps.
We focus here on the more interesting scenarios with two or more related targets,
in which case one may wish to study the progress of individuals to those targets jointly rather than separately.

To study progression with respect to two or more related targets,
we extend the latent process model of Section \ref{sec:one} as follows.
Consider two related targets centered at $\mT_1 \in \mR^q$ and $\mT_2 \in \mR^q$ (e.g., algebra and geometry).
Assume that two sets of variables are available for measuring progress towards targets $\mT_1$ and $\mT_2$,
and that the positions of those two sets of variables with positions 
\beno
\bm{b}_j &\iid& \mbox{MVN}_q(\mT_1,\, \sigma_B^2\, \bm{I}_q)
\ee
and
\beno
\bm{b}_j &\iid& \mbox{MVN}_q(\mT_2,\, \sigma_B^2\, \bm{I}_q),
\ee
respectively,
where \sigma_B\, >\, 0$.

As before,
we assume that the position $\bm{a}_{i,1}$ of individual $i$ at time $t=1$ is generated from 
\beno
\bm{a}_{i,t} &\iid& \mbox{MVN}_q(\mT,\, \bSigma_A),
&& \bSigma_A\, \succ\, 0.
\ee
We assume that individual $i$'s position $\bm{a}_{i,t}$ at time $t \geq 2$ is determined as follows.
First,
we assume that individual $i$ moves towards a target $\mC_{i,t} \in \mR^q$.
The target $\mC_{i,t} \in \mR^q$ is a convex combination of two related targets $\mT_1 \in \mR^q$ and $\mT_2 \in \mR^q$:
\be
\mC_{i,t} \;=\; (1-\omega_{i,t})\; \mT_1 + \omega_{i,t}\; \mT_2,
&& t = 2, \dots, T,
\ee
where the parameter $\omega_{i,t} \in [0, 1]$ determines whether individual $i$ is on the shortest path towards making progress on target $\mT_1$ ($\omega_{i,t}=0$) or target $\mT_2$ ($\omega_{i,t}=1$) or makes progress with respect to both targets.
Second,
the position $\bm{a}_{i,t}$ of individual $i$ at time $t$ is determined as follows:
\beno
\bm{a}_{i,t}
&=& (1-\lambda_{i,t})\; \bm{a}_{i,t-1} + \lambda_{i,t}\; \mC_{i,t-1},
&& t = 2, \dots, T.
\ee
The parameter $\lambda_{i,t} \in [0, 1]$ can be interpreted as the rate of progress of individual $i$ towards target $\mC_{i,t}$ between time $t-1$ and $t$:
If $\lambda_{i,t} = 0$,
individual $i$ makes no progress towards target $\mC_{i,t}$,
whereas $\lambda_{i,t} = 1$ implies that individual $i$ reaches target $\mC_{i,t}$ by time $t$.
A visual representation of the latent process can be found in Figure \ref{fg:target2}.

\begin{figure}[t]
\centering

\begin{tikzpicture}
[scale=.75, 
  transform shape, node distance=2cm,
  roundnode/.style={circle, draw=black, thick, minimum size=10mm},
  squarednode/.style={rectangle, draw=black, thick, minimum size=6mm},
  arrow/.style = {semithick,-Stealth},
  roundnode/.style={rectangle,draw=black, sep=0pt,minimum minimum size = 10mm,circle} % <- this is new
]

% x axis 
\draw   (0,0) -- (12, 0) ;
% y axis 
\draw   (0,0) -- (0,8) ;

% variable groups 
\draw[fill=green!20,draw=none]  (3,6) circle (1.2cm) node [scale=1.2] {$\mT_1$} ; 
\draw[fill=blue!20,draw=none]  (10,5) circle (1.2cm) node [scale=1.2] {$\mT_2$} ; 



% variables in group A 


\draw [fill] (2.9,6.5) circle (.6mm)     ;
\draw [fill] (2.6,5.5) circle (.6mm)     ;
\draw [fill] (3.5,5.9) circle (.6mm)     ;

% variables in group B
\draw [fill]  (9.9,5.5) circle (.6mm)     ;
\draw [fill] (9.6,4.5) circle (.6mm)    ;
\draw [fill] (9.5,4.9) circle (.6mm)    ;

% person 2 time 1 
\draw [fill] (7,1) circle (1mm)  ;
\draw (7,.5) node [scale=1.2] {$\bm{a}_{i,1}$} ;


% path for person 2 toward A 
\draw [->,dashed] (7,1) -- (3,5.8); 
%\draw[->, thick,dashed] (6,1) -- (3.1,3.3); 

% path for person 2 toward G
\draw [->,dashed] (7,1) -- (10,4.8); 

% path between A and G
\draw [dashed] (3.2,6) -- (9.8,5); 


% person 2 time 2 
\draw [fill] (5.7,4) circle (1mm)  ;
\draw (5.1,4) node [scale=1.2] {$\bm{a}_{i,2}$} ;

% movement 
\draw[->,dashed, thick] (7,1) -- (5.7,3.9); 

% to the top
\draw[dashed, thick] (5.7,3.9) -- (5,5.6); 
\draw[fill]  (5,5.7) circle (1mm)  ;
\draw (4.7,6.3) node [scale=1.2] {$\mC_{i,t}$} ;


% i1=i2
\draw (7,1) to [out=30,in=30] (5.7,4) ; 
\draw (6.8,2.6) node [scale=1.2] {$\lambda_{i,t}$} ;

% c-M 
%\draw (5,5.7) to [out=40,in=120] (10,5) ; 
%\draw (7.3,6) node [scale=1.2] {$\omega_{i,t}$} ;

\end{tikzpicture}

\caption{an individual $i$ makes progress towards target $\mC_{i,t} \in \mR^2$,
which is a convex combination of targets $\mT_1 \in \mR^2$ and $\mT_2 \in \mR^2$.
The shaded balls centered at $\mT_1$ and $\mT_2$ indicate the sets of variables that measure the two targets.}
\label{fg:target2}
\end{figure}

}

\subsection{Priors}
\label{sec:prior}

Since the weights $\alpha_{i,t}$,
$\beta_{j,t}$,
and $\gamma$ cannot be all estimated,
we assume that $\alpha_{i,t} = 0$ with probability $1$ and $\beta_{j,t} \mid \sigma_\beta^2\; \iid\; N(0,\, \sigma_\beta^2)$ and $\gamma \mid \sigma_\gamma^2$ $\sim$ Half-Normal$(0,\, \sigma^2_\gamma)$,
where $\sigma_\beta^2 > 0$ and $\sigma_\gamma^2 > 0$.
% are specified hyperparameters.
We review identifiability issues in Section \ref{sec:id}.

If there are no predictors of the rates of progress $\lambda_{i,t}$,
a flexible prior of $\lambda_{i,t}$ is specified by
\beno
\logit(\lambda_{i,t})
\mid \pi_{i,t},\, \mu_0,\, \sigma_0^2,\, \mu_1,\, \sigma_1^2
&\ind& (1-\pi_{i,t})\; N(\mu_0,\, \sigma_0^2) + \pi_{i,t}\; N(\mu_1,\, \sigma_1^2),
\ee
where $\pi_{i,t} \in (0,\, 1)$ are mixing proportions,
while $(\mu_0,\, \sigma_0^2) \in \mR \times (0,\, +\infty)$ and $(\mu_1,\, \sigma_1^2) \in \mR \times (0,\, +\infty)$.
% are specified hyperparameters.
The hyperparameters are chosen so that the distribution of $\lambda_{i,t}$ is a mixture of two distributions,
one of them placing 95\% of its mass between .01 and .21 and the other placing 95\% of its mass between .04 and .96.
The two-component mixture prior of $\lambda_{i,t}$ is motivated by the observation that,
more often than not,
some individuals make negligible progress while others make non-negligible progress.
A plot of the two-component mixture prior of $\lambda_{i,t}$ can be found in Supplement \ref{mixture_prior}. 
The mixing proportions $\pi_{i,t}$ have priors $\pi_{i,t} \mid a_\pi,\, b_\pi\, \iid\, \mbox{Beta}(a_\pi,\, b_\pi)$,
where $a_\pi > 0$ and $b_\pi > 0$.
% are specified hyperparameters.

If there are predictors of the rates of progress $\lambda_{i,t}$,
the prior of the predictor weights $\delta_{0,t}, \dots, \delta_{w,t}$ is a spike-and-slab distribution,
which encourages sparsity.

Additional details on the priors can be found in Supplement \ref{appendix:estimation}.

\subsection{Identifiability issues}
\label{sec:id}

The latent process model has the same identifiability issues as latent space models in statistical network analysis \citep[e.g.,][]{Hoff:2002,ScSn03,HaRaTa07,sewell2015latent,SmAsCa19},
because the Euclidean distances $d(\bm{a}_{i,t}, \mT)$ are invariant to reflection,
translation, 
and rotation of the positions $\bm{a}_{i,t}$ of individuals $i$ at time $t$ and target $\mT$.
We address these issues by basing statistical inference on equivalence classes of positions,
using Procrustes matching \citep{Hoff:2002}.

A second issue is that the weights $\alpha_{i,t}$,
$\beta_{j,t}$,
and $\gamma$ cannot be all estimated:
e.g.,
for all $c \in \mR$,
\beno
\eta_{i,j,t}(\mu_{i,j,t}(\btheta,\,  \bm{a}_{i,t},\, \mT)) 
&=& (\alpha_{i,t} - c) + (\beta_{j,t} + c) + \gamma\; g(\bm{a}_{i,t},\, \mT).
% \\
% &=& (\alpha_{i,t} - c) + \beta_{j,t} + (\gamma\; g(\bm{a}_{i,t},\, \mT) - c).
% \;=\; \alpha_{i,t} + (\beta_{j,t} - c) + (\gamma\; g(\bm{a}_{i,t}, \mT) + c).
\ee
We hence assume that $\alpha_{i,t} = 0$ with probability $1$ while $\beta_{j,t} \mid \sigma_\beta^2\; \iid\; N(0,\, \sigma_\beta^2)$ and $\gamma \mid \sigma_\gamma^2$ $\sim$ Half-Normal$(0,\, \sigma^2_\gamma)$,
where $\sigma_\beta^2 > 0$ and $\sigma_\gamma^2 > 0$.
% are specified hyperparameters.
Setting $\alpha_{i,t} = 0$ is convenient,
because the distance term $\gamma\, g(\bm{a}_{i,t}, \mT)$ helps quantify the rate of progress of individual $i$ towards target $\mT$ and is hence more interesting than the individual weight $\alpha_{i,t}$.

A third issue is that the weight $\gamma$ of the distance function $g(\bm{a}_{i,t}, \mT)$ is not identifiable:
e.g.,
for all $c > 0$,
\beno
\eta_{i,j,t}(\mu_{i,j,t}(\btheta,\,  \bm{a}_{i,t},\, \mT)) 
% &\coloneqq& \beta_{j,t} + \gamma\, \exp(- d(\bm{a}_{i,t}, \mT))\s
% \\
&=&  \beta_{j,t} + (\gamma\, \exp((c-1)\, d(\bm{a}_{i,t}, \mT)))\, \exp(- d(c\, \bm{a}_{i,t},\, c\, \mT)).
\hide{
&=& (\gamma\, \exp((c-1)\, |\!|\bm{a}_{i,t} - \mT |\!|_2)))\, \exp(- c\, |\!|\bm{a}_{i,t} - \mT |\!|_2)\s
\\
}
\ee
These identifiability issues can be addressed by constraining the positions $\bm{a}_{i,t}$ of individuals $i$ at time $t$ and target $\mT$.
Details are provided in Supplement \ref{appendix:mcmc}. % \ref{appendix:estimation}.

\subsection{Comparison}
\label{sec:comparison}

We compare the latent process model with the classic model of \citet{andersen:85},
which assumes that responses $Y_{i,j,t} \in \{0, 1\}$ are independent $\mbox{Bernoulli}(\mu_{i,j,t})$ ($\mu_{i,j,t} \in (0, 1)$) random variables with $\logit(\mu_{i,j,t}) = \beta_j + \vartheta_{i,t}$.

To facilitate comparisons,
we focus on responses $Y_{i,j,t} \in \{0, 1\}$ at times $t \in \{1, 2\}$ and one of the simplest specifications of the latent process model,
with a logit link function,
time-invariant weights $\beta_{j,1} = \beta_{j,2} = \beta_j$, 
and a distance function of the form $g(\bm{a}_{i,t}, \mT) \coloneqq d(\bm{a}_{i,t}, \mT)$ with weight $\gamma = -1$.
The negative distance function is a simple and convenient choice that facilitates comparisons,
although it is less interpretable than other specifications of the distance function,
as discussed in Section \ref{sec:data.model}.

The latent process model with a logit link function and a negative distance function is equivalent to the $\logit(\mu_{i,j,t}) = \beta_j + \vartheta_{i,t}$ model with parameters $\beta_{j,1} = \beta_{j,2} = \beta_j$ and
\be
\label{varthetas}
\vartheta_{i,1}
&=& -d(\bm{a}_{i,1},\, \mT)\s
\\
\vartheta_{i,2}
&=& -d(\bm{a}_{i,2},\, \mT)
\;\;=\;\; - (1 - \lambda_{i,2})\; d(\bm{a}_{i,1},\, \mT)
\;\;=\;\; (1 - \lambda_{i,2})\; \vartheta_{i,1}.
\ee
Thus,
the rate of progress $\lambda_{i,2}$ of individual $i$ between time $1$ and $2$ is
\beno
\lambda_{i,2}
&=& 1 - \dfrac{\vartheta_{i,2}}{\vartheta_{i,1}},
\ee
where $\lambda_{i,2} \in [0, 1]$ provided $\vartheta_{i,1} \leq \vartheta_{i,2}$;
note that $\vartheta_{i,1} \leq 0$ and $\vartheta_{i,2} \leq 0$ by equation \eqref{varthetas}.
In other words,
the higher $\vartheta_{i,2}$ is relative to $\vartheta_{i,1}$,
the higher is the rate of progress $\lambda_{i,2}$.

As a consequence,
the latent process model with a negative distance function can be viewed as a geometric version of \citeauthor{andersen:85}'s classic model,
with the advantage of providing an embedding of both individuals and the target of interest in a shared metric space.
In addition,
the latent process model quantifies the rate of progress of individual $i$ by a real number between $0$ (no progress) and $1$ (target reached),
rather than a difference of the form $\vartheta_{i,2} - \vartheta_{i,1}$ (which can be arbitrarily large).
Last,
but not least,
the latent process model helps quantify how much more progress individuals can make in the future,
because the rate of progress $\lambda_{i,2}$ is bounded above by $1$ (target reached).

It is worth noting that the latent process model assumes that individuals either make no progress at all or make some progress,
but it does not allow individuals to regress (the opposite of progress).
The logit model does allow individuals to regress.
While the latent process model can be extended to capture regress,
we focus here on progress, 
motivated by the applications in Sections \ref{sec:math} and \ref{sec:coursekata}. 

\section{Bayesian inference}
\label{sec:inference}

Consider the latent process model without predictors of the rates of progress $\lambda_{i,t}$ and define $\bm{y} \coloneqq (y_{i,j,t})_{1 \leq i \leq n,\, 1 \leq j \leq p,\, 1 \leq t \leq T}$,\,
$\bm\beta \coloneqq (\beta_{j,t})_{1 \leq j \leq p,\, 1 \leq t \leq T}$,\break
$\bm\lambda \coloneqq (\lambda_{i,t})_{1 \leq i \leq n,\, 2 \leq t \leq T}$,
$\bm\pi \coloneqq (\pi_{i,t})_{1 \leq i \leq n,\, 2 \leq t \leq T}$,\,
$\bm{A} \coloneqq (\bm{a}_{i,t})_{1 \leq i \leq n,\, 1 \leq t \leq T}$,\,
and\break
$\bm{B} \coloneqq (\bm{b}_{j,t})_{1 \leq j \leq p,\, 1 \leq t \leq T}$.
Then the posterior is proportional to
\beno
f(\bm\beta,\, \gamma,\, \bm{A},\, \bm{B},\, \mT,\, \bm\lambda,\, \bm\pi \mid \bm{y})
\;\propto\; \left[\dprod_{i=1}^n\, \dprod_{j=1}^{p}\, \dprod_{t=1}^T f(y_{i,j,t} \mid \beta_{j,t},\, \gamma,\, \bm{a}_{i,t},\, \mT)\right]\s
\\
\times\; \left[\, \dprod_{i=1}^n\, f(\bm{a}_{i,1})\, \dprod_{t=2}^T\, f(\bm{a}_{i,t} \mid \bm{a}_{i,t-1},\, \mT,\, \lambda_{i,t})\right]\, \times\, \left[\, \dprod_{j=1}^p\, f(\bm{b}_j \mid \mT)\right] \times\, f(\mT)\s
\\
\times\; \left[\, \dprod_{i=1}^n\, \dprod_{t=2}^T\, f(\lambda_{i,t} \mid \pi_{i,t})\; f(\pi_{i,t})\right] \times \left[\, \dprod_{j=1}^p\, \dprod_{t=1}^T\, f(\beta_{j,t})\right] \times\, f(\gamma),
\ee
where,
in an abuse of notation, 
$f$ denotes a probability mass or density function with suitable support.
It is worth noting that the conditional densities $f(\bm{a}_{i,t} \mid \bm{a}_{i,t-1},\, \mT,\, \lambda_{i,t})$ are point masses,
because the positions $\bm{a}_{i,t} \coloneqq (1-\lambda_{i,t})\; \bm{a}_{i,t-1} + \lambda_{i,t}\; \mT$ are non-random functions of $\bm{a}_{i,t-1}$ and $\lambda_{i,t}$ for fixed $\bm{a}_{i,t-1}$ and $\lambda_{i,t}$ ($t = 2, \dots, T$).

We approximate the posterior by Markov chain Monte Carlo:
e.g.,
if all responses $Y_{i,j,t} \in \{0, 1\}$ are binary,
we use the P\'{o}lya-Gamma sampler of \citet{polson:13} for updating unknown quantities in the data model and Gibbs samplers and Metropolis-Hasting steps for updating unknown quantities in the process model.
Details are provided in Supplement \ref{appendix:mcmc}.


==> old/posterior.tex <==
\beno
f(\bm\alpha,\, \bm\beta,\, \gamma,\, \bm{A},\, \bm{B},\, \bm\lambda,\, \bm\pi \mid \bm{y})
&\propto& \left[\dprod_{i=1}^n\, \dprod_{j=1}^{p}\, \dprod_{t=1}^T f(y_{i,j,t} \mid \alpha_{i,t},\, \beta_{j,t},\, \gamma,\, \bm{a}_{i,t},\, \bm{b}_1, \dots, \bm{p}_p)\right]\s
\\
&\times& \left[\, \dprod_{i=1}^n\, \dprod_{t=1}^T\, f(\alpha_{i,t})\right]
\times \left[\, \dprod_{j=1}^p\, \dprod_{t=1}^T\, f(\beta_{j,t})\right] \times\, f(\gamma)\s
\\
&\times& \left[\, \dprod_{i=1}^n\, f(\bm{a}_{i,1})\, \dprod_{t=2}^T\, f(\bm{a}_{i,t} \mid \bm{a}_{i,t-1},\, \bm{b}_1, \dots, \bm{p}_p,\, \lambda_{i,t})\right] \times \left[\, \dprod_{j=1}^p\, f(\bm{b}_j)\right]\s
\\
&\times& \left[\, \dprod_{i=1}^n\, \dprod_{t=2}^T\, f(\lambda_{i,t} \mid \pi_{i,t})\; f(\pi_{i,t})\right]
\ee


==> other.approaches.first.tex <==
\subsection{Other possible approaches to measuring progress}
\label{sec:other.approaches}

There are other possible approaches to measuring progress,
both within and outside of the proposed statistical framework.

To demonstrate, 
recall that the proposed statistical framework builds on generalized linear models.
In other words,
the responses $Y_{i,j,t}$ have exponential-family distributions $\mbP_{\btheta,\bm{a}_{i,t},\bm{b}_j}$ \citep{Su19,efron22}.
In the language of exponential families,
the proposed statistical framework measures progress based on the canonical parameterization of the exponential family.
An alternative would be to measure progress based on the mean-value parameterization of the exponential family.

To compare these alternative approaches to assessing progress,
let $\bm{Y}_i \coloneqq (Y_{i,j,t})_{1 \leq j \leq p,\, 1 \leq t \leq T}$\, be the vector of responses $Y_{i,j,t}$ of individual $i$ and let the distributions $\mbP_{\btheta,\bm{a}_{i,t},\bm{b}_j}$ of responses $Y_{i,j,t}$ be one-parameter exponential-family distributions (e.g., $Y_{i,j,t} \mid \mu_{i,j,t}$ $\ind$ $\mbox{Bernoulli}(\mu_{i,j,t})$ with mean $\mu_{i,j,t} \in (0, 1)$,\,
$Y_{i,j,t} \mid \mu_{i,j,t}\; \ind\; \mbox{Poisson}(\mu_{i,j,t})$ with mean $\mu_{i,j,t} \in (0, +\infty)$,\,
or $Y_{i,j,t} \mid \mu_{i,j,t},\, \sigma_{i,j,t}^2\; \ind\; N(\mu_{i,j,t},\, \sigma_{i,j,t}^2)$ with mean $\mu_{i,j,t} \in \mR$ and known variance $\sigma_{i,j,t}^2 \in (0, +\infty)$).
Then the probability density function of an exponential-family probability measure $\mbP_{\btheta,\bm{a}_{i,t},\bm{b}_j}$ dominated by a $\sigma$-finite measure $\nu$ can be represented as
\beno
f(y_{i,j,t} \mid \eta_{i,j,t})
&=& a_{i,j,t}(y_{i,j,t})\,  \exp(\eta_{i,j,t}\, s_{i,j,k}(y_{i,j,t}) - \psi_{i,j,t}(\eta_{i,j,t})),
\ee
where $a_{i,j,t}(y_{i,j,t}) \in [0, +\infty)$ is a function of $y_{i,j,t}$,\,
$\eta_{i,j,t} \equiv \eta_{i,j,t}(\mu_{i,j,t}(\btheta,\, \bm{a}_{i,t},\, \bm{b}_j)) \in \mR$ is a canonical parameter,
$s_{i,j,t}(y_{i,j,t}) \in \mR$ is a sufficient statistic,
and
\beno
\psi_{i,j,t}(\eta_{i,j,t})
&\coloneqq& \dint_{\mY_{i,j,t}} \exp(\eta_{i,j,t}\, s_{i,j,k}(y_{i,j,t})) \dd \nu(y_{i,j,t})
\ee
ensures that $f(y_{i,j,t} \mid \eta_{i,j,t})$ integrates to $1$;
note that the general formulation above covers both the discrete setting (in which case $\nu$ may be counting measure) and the continuous setting (in which case $\nu$ may be Lebesgue measure).
As a result,
the probability density function of the response vector $\bm{Y}_i$ of individual $i$ can be represented as
\beno
f(\bm{y}_i \mid \bm\eta_i)
&=& \dprod_{j=1}^p\, \dprod_{t=1}^T f(y_{i,j,t} \mid \eta_{i,j,t})
&=& a_i(\bm{y}_i)\, \exp\left(\langle\bm\eta_i, s_i(\bm{y}_i)\rangle - \psi_i(\bta_i)\right),
\ee
where $a_i(\bm{y}_i) \coloneqq \prod_{j=1}^p \prod_{t=1}^T a_{i,j,t}(y_{i,j,t})$,\,
$\psi_i(\bta_i) \coloneqq \sum_{j=1}^p \sum_{t=1}^T \psi_{i,j,t}(\eta_{i,j,t})$,\,
and $\langle\bm\eta_i, s_i(\bm{y}_i)\rangle$ denotes the inner product of the vector of canonical parameters $\bm\eta_i \coloneqq (\eta_{i,j,t})_{1 \leq j \leq p,\, 1 \leq t \leq T}$ and the vector of sufficient statistics $s_i(\bm{y}_i) \coloneqq (s_{i,j,t}(y_{i,j,t}))_{1 \leq j \leq p,\, 1 \leq t \leq T}$.
In other words,
if the responses $Y_{i,j,t}$ have exponential-family distributions,
so does the response vector $\bm{Y}_i$ of individual $i$.
The parameter vector 
\beno
\bm\mu_i(\bm\eta_i) 
&\coloneqq& \mbE_{\bm\eta_i}\, s_i(\bm{Y}_i)
\ee
with coordinates $\mu_{i,j,t}(\bm\eta_i) \coloneqq \mbE_{\bm\eta_i}\, s_{i,j,t}(Y_{i,j,t})$ is known as the mean-value parameter vector of the exponential family.
Since the map $\bm\eta_i \mapsto \bm\mu_i(\bm\eta_i)$ is a homeomorphism and is hence one-to-one \citep[][Theorem 3.6, p.\ 74]{Br86},
one can parameterize the model by using either the canonical parameter vector $\bm\eta_i$ or the mean-value parameter vector $\bm\mu_i(\bm\eta_i)$.
As a consequence,
one can measure progress based on either the canonical parameterization or the mean-value parameterization:
e.g.,
if the responses $Y_{i,j,t}$ of individual $i$ to variables $j$ have been recorded at $T = 2$ time points,
one could measure progress based on differences in mean-value parameters $\mu_{i,j,2}(\bm\eta_i)$ and $\mu_{i,j,1}(\bm\eta_i)$,
summed over all variables $j$:
\beno
\mbox{progress of individual $i$} 
&\coloneqq& \dsum_{j=1}^p \left[\mu_{i,j,2}(\bm\eta_i) - \mu_{i,j,1}(\bm\eta_i)\right].
\ee
In addition,
one could assess how much more progress individual $i$ can make in the future:
\beno
\mbox{possible progress of individual $i$ in the future}
&\coloneqq& \dsum_{j=1}^p \left[\sup\limits_{\bm{\eta}_i}\, \mu_{i,j,2}(\bm\eta_i) - \mu_{i,j,2}(\bm\eta_i)\right].
\ee
That being said,
the mean-value parameterization is less convenient for the purpose of model selection,
e.g.,
the problem of determining whether students make progress.
In fact,
it is common practice to base model selection of generalized linear models on the canonical parameterization rather than the mean-value parameterization of exponential families.
Therefore,
we assess whether and how much progress individuals $i$ make towards the target of interest $\mT$ based on the canonical parameterization rather than the mean-value parameterization.
The resulting statistical framework comes with the benefit of model selection (e.g., determining whether individuals make progress) and inherits the advantages of the \citet{jeon:21} model,
which is likewise based on the canonical parameterization rather than the mean-value parameterization.


==> plot_test.tex <==

\begin{figure}[t]
\begin{center}
\begin{tikzpicture}
[scale=4, 
  transform shape, node distance=2cm,
  roundnode/.style={circle, draw=black, thick, minimum size=10mm},
  squarednode/.style={rectangle, draw=black, thick, minimum size=6mm},
  arrow/.style = {semithick,-Stealth},
  dotnode/.style={fill,inner sep=0pt,minimum size=2pt,circle} 
]


% x axis 
\draw   (-1.2,0) -- (1.1, 0) ;
% y axis 
\draw   (0,-1) -- (0,1) ;

% Target:
\draw [fill=green!10,draw=none] (0.024 ,0.040) circle (0.1cm) node [scale=0.5]  {$\mT$} ; % 

% % Original position of student A at t1:
% \draw [fill] (-3.311 , -1.614) circle (1mm)  ;
% \draw (-3.71 , -1.61) node [scale=1.5] {$A$}; 

% % person A t2 
% \draw [fill] (-0.428, -0.033) circle (1mm)  ;
% \draw[->, thick,dashed] (-3.31 , -1.61)  -- (-0.628, -0.033); 

% Original position of student A at t1:
\draw [fill] (0.509 , -0.530) circle (0.3mm)  ;
\draw (0.709 , -0.530) node [scale=0.5] {$A$}; 

% person A t2 
\draw [fill] ( 0.130, -0.102) circle (0.3mm)  ;
\draw[->, thick,dashed] (0.509 , -0.530)  -- (0.130, -0.102); 




% person B t1
\draw [fill] (-0.741, 0.572) circle (0.3mm)  ;
\draw (-0.941, 0.572) node [scale=0.5] {$B$} ;

% person B t2 
\draw [fill] (-0.150, 0.177) circle (0.3mm)  ;
\draw[->, thick,dashed] (-0.741, 0.572)   -- (-0.150, 0.177)  ; 



% % person C t1
% \draw [fill] (1.733, -0.148) circle (1mm)  ;
% \draw (2.133, -0.148) node [scale=1.5] {$C$} ; 

% % person C t2 
% \draw [fill] (0.7884 ,-0.006) circle (1mm)  ;
% \draw[->, thick,dashed] (1.733, -0.148)  -- (0.8884 ,-0.006)   ; 


% person C t1
\draw [fill] ( 0.078 , 0.629) circle (0.3mm)  ;
\draw (0.278 , 0.629) node [scale=0.5] {$C$} ; 

% person C t2 
\draw [fill] (  0.060, 0.274) circle (0.3mm)  ;
\draw[->, thick,dashed] ( 0.078 , 0.629)  -- (0.060, 0.274) ; 


% % person D t1
% \draw [fill] (-4.032 ,1.727) circle (1mm)  ;
% \draw (-4.432 ,1.727) node [scale=1.5] {$D$} ; 

% % person D t2 
% \draw [fill] (-0.563, 0.388) circle (1mm)  ;
% \draw[->, thick,dashed] (-4.032 ,1.727)  -- (-0.763, 0.388) ; 


% person D t1
\draw [fill] (1.002 ,-0.531) circle (0.3mm)  ;
\draw (1.202 ,-0.531) node [scale=0.5] {$D$} ; 

% person D t2 
\draw [fill] (0.273,-0.090) circle (0.3mm)  ;
\draw[->, thick,dashed] (1.002 ,-0.531)  -- (0.273,-0.090) ; 



\end{tikzpicture}
\end{center}
\caption{An embedding of Hispanic students $A$, $B$, $C$, and $D$ along with learning target $\mT$,
the understanding of numbers and arithmetic operations,
into $\mR^2$.
% the metric space $(\mathbb{M}, d)$ consisting of the two-dimensional Euclidean space $\mathbb{M} \coloneqq \mR^2$ equipped with the Euclidean norm $d(\bm{a}, \bm{b}) \coloneqq |\!|\bm{a} - \bm{b}|\!|_2$ ($\bm{a} \in \mR^2$, $\bm{b} \in \mR^2$).
These results are based on a Bayesian approach to the proposed latent process model,
using data collected on the online learning platform My Math Academy.
The posterior medians of the positions of students $A$, $B$, $C$, and $D$ at the first and second test are represented by circles and connected by arrows.
The results reveal that some students made more progress than others and that students $A$ and $D$ may be close to reaching the target, while student $B$ and $C$ may need additional assistance.
% Note that the distances between the students and the target $\mT$ affect the responses of students,
% but the distances between the students do not affect the responses.
\label{examplefigure}}
\end{figure}

==> simulation_new.tex <==




\subsection{New Simulation Results}

We consider a situation where $n=60$ individuals worked on $p=20$ problems at each of two time points 1 and 2. We assume three groups of individuals, 20 per group, with different progress rates with no progress, medium progress, and large progress. Importantly, we assume the difficulty of the items change from time point 1 to time point 2. 
We consider two cases where the problems become easier (condition 1) and the problems become more difficult (condition 2). 
To generate data from these scenarios, we use the logit model in Equation (\ref{eq:logit}). Data generating values are shown in Table \ref{tab:data_gen}. 
We generate 300 data sets per condition and fit three models to the simulated data sets: the proposed model, the logit model with the sign and order constraints on $\zeta_{i,t}$ and the standard logit model with no constraints. All three models are estimated using MCMC. 


\begin{table}[]
    \centering
\begin{tabular}{c|cc| cc| cc}
\hline 
                & group 1 &  & group 2 && group 3 \\
\hline 

                & T1 & T2 &  T1 & T2  & T1 & T2 \\ 
\hline 
Condition 1 && &&  && \\ 
$\beta_{j,t}$  &  0  & 0 & 0  & 0&  0  & 0 \\
$\zeta_{j,t}$  &  -2 & -2 & -2 & 0 & -2 & 2 \\  
\hline 
Condition 2 && &&  && \\ 
$\beta_{j,t}$  &  0  & 1 & 0  & 1 &  0  & 1 \\
$\zeta_{j,t}$  &  -2 & -2 & -2 & 0 & -2 & 2 \\  
\hline 
Condition 3 && &&  && \\ 
$\beta_{j,t}$  &  0  & -1 &  0  & -1 &  0  & -1 \\
$\zeta_{j,t}$  &  -2 & -2 & -2 & 0 & -2 & 2 \\  
\hline 
\end{tabular}
    \caption{Data generating values for the three conditions}
    \label{tab:data_gen}
\end{table}



\begin{table}[]
    \centering
\begin{tabular}{c|cc| cc| cc}
\hline 
                & group 1 &  & group 2 && group 3 \\
\hline 

                & T1 & T2 &  T1 & T2  & T1 & T2 \\ 
\hline 
Condition 1 && &&  && \\ 
$\beta_{j,t}$  &  0  & 0 & 0  & 0&  0  & 0 \\
$\zeta_{j,t}$  &  -2 & -2 & -2 & 0 & -2 & 2 \\  
\hline 
Condition 2 && &&  && \\ 
$\beta_{j,t}$  &  0  & 1 & 0  & 1 &  0  & 1 \\
$\zeta_{j,t}$  &  -2 & -2 & -2 & 0 & -2 & 2 \\  
\hline 
Condition 3 && &&  && \\ 
$\beta_{j,t}$  &  0  & -1 &  0  & -1 &  0  & -1 \\
$\zeta_{j,t}$  &  -2 & -2 & -2 & 0 & -2 & 2 \\  
\hline 
\end{tabular}
    \caption{Michael: Data generating values for the three conditions}
    \label{tab:data_gen}
\end{table}



\begin{figure}[hptb]
    \centering
     \includegraphics[width=0.3 \textwidth]{figure/sim_diff_0_med.pdf} 
          \includegraphics[width=0.3 \textwidth]{figure/sim_diff_1_med.pdf} 
               \includegraphics[width=0.3 \textwidth]{figure/sim_diff_3_med.pdf} 
   \caption{
  (a) condition 1:  problem difficulty stays the same 
  (b) condition 2: problems get easier at time 2 
  (c) condition 3: problems  get more difficulty at time 2 
   }
   \label{fg:sim1}
\end{figure}      


\begin{figure}[hptb]
    \centering
     \includegraphics[width=0.3 \textwidth]{figure/beta_cond1.pdf} 
          \includegraphics[width=0.3 \textwidth]{figure/beta_cond2.pdf} 
               \includegraphics[width=0.3 \textwidth]{figure/beta_cond3.pdf} 
   \caption{
  (a) condition 1:  problem difficulty stays the same 
  (b) condition 2: problems get easier at time 2 
  (c) condition 3: problems  get more difficulty at time 2 
   }
   \label{fg:sim1}
\end{figure}      



==> title.figure4.tex <==
Histogram of the posterior medians of rates of progress $\lambda_i$ of individuals $i$. 
For each individual $i$,
the mean of 250 posterior medians of $\lambda_i$ based on 250 simulated data sets is plotted.


==> trash <==
\hide{
\begin{enumerate}
\item The classic approach to assessing progress based on \citeauthor{andersen:85}'s (\citeyear{andersen:85}) model and its extensions helps estimate how much progress individuals $i$ make (model estimation),
but does not determine whether individuals $i$ make progress (model selection).
By contrast,
the proposed latent process model does double duty:
It helps determine whether individuals $i$ make progress (model selection),
in addition to estimating how much progress individuals $i$ make (model estimation),
and how much more progress individuals $i$ can make in the future.
\end{enumerate}
}

\hide{
The motivating example demonstrates that the proposed latent process model has at least three advantages:
(a) it provides a geometric summary of progress towards a target of interest in a low-dimensional Euclidean space;
(b) it helps detect individuals who need more assistance than others;
and (c) it helps quantify how much room is left for improvement.
}

\hide{
A metric space $(\mathbb{M},\, d)$ consists of a space $\mathbb{M}$ and a distance function $d: \mathbb{M}^2 \mapsto [0, +\infty)$ satisfying
\bi
\item reflexivity: $d(\bm{a},\, \bm{b}) = 0$ if and only if $\bm{a} = \bm{b} \in \mathbb{M}$;
\item symmetry: $d(\bm{a},\, \bm{b}) = d(\bm{b},\, \bm{a})$ for all $(\bm{a},\, \bm{b}) \in \mathbb{M}^2$;
\item the triangle inequality: $d(\bm{a},\, \bm{b}) \leq  d(\bm{a},\, \bm{c}) + d(\bm{b},\, \bm{c})$ for all $(\bm{a},\, \bm{b},\, \bm{c}) \in \mathbb{M}^3$.
\ei
}

\hide{
A second example is the challenge of assessing whether individuals progress or regress:
e.g.,
when patients are treated for depression,
some patients may first become more depressive,
and then less depressive.
}

\hide{
A theoretical advantage is that the latent process models has additional structure in the form of a metric space.
Additional structure is important,
because many item response models have individual-specific parameters and have therefore more parameters than observations.
It is well-known that consistent estimation of statistical exponential-family models --- including the longitudinal item response model described above --- is possible when the number of parameters $s$ satisfies $s \ll n$ \citep[e.g.,][]{Po88},
but may require additional structure when $s \gg n$ \citep[e.g., sparsity,][]{Wa19}:
e.g.,
the longitudinal item response model described above has $s = (p + n)\, T > n$ parameters and may therefore benefit from additional structure.
The proposed latent process model provides additional structure in the form of a metric space that can facilitate statistical inference,
in addition to having practical advantages (as described above).
}


\hide{
Examples of discrete latent variable models include longitudinal diagnostic classification analysis (reference);
latent transition variable response analysis (reference);
and latent class target progression methods (references).
These approaches measure progress based on changes in the classification of students,
e.g.,
based on whether students transition from a subset of skilled students to a subset of non-skilled students.
That said,
classifications of students into two or more subsets of students (e.g., skilled versus non-skilled students) may be too coarse to capture individual differences in learning progress.
While some models --- e.g., longitudinal mixture variable response models --- do allow for individual differences among students within subsets of students,
they share the same disadvantages as continuous latent variable approaches.
}

\hide{

\subsection{Existing methods}

The idea of embedding data into Euclidean space has a long history in educational statistics and related areas,
as demonstrated by multidimensional scaling \citep[e.g.,][]{To52,Tw65,Oh:2001,Oh:2007}.
In recent decades,
the idea of embedding data into Euclidean space has been adapted to network data represented by a graph with connections among nodes: see, e.g., \cite{Hoff:2002,ScSn03,Handcock:2007, Krivitsky:2009, Raftery:2012, Sweet:13, STMu13,TaSuPr13,SuTaPr14,sewell2015latent,Rastelli:2015,SmAsCa19};
and \cite{MaMaYu20}. 
Our innovation comes from that we capture individual students' learning progress to targets based on their movements in a low-dimensional geometric space.
To the best of our knowledge,
nothing comparable has not been attempted before.
Here we review some existing methods to evaluate students' growth over time. %
}

\hide{
We consider online educational data in the form of $p \in \{1, 2, \dots\}$ problems.
If $p$ is large,
the problems may be divided into subsets of problems.
We consider problems partitioned into $K \in \{2, 3, \dots\}$ non-empty and non-overlapping subsets of problems $\mB_1, \dots, \mB_K$,
which may correspond to the chapters of a book with $K$ chapters.
The number of problems may vary from chapter to chapter.
Suppose that $n \in \{1, 2, \dots\}$ test takers solve one or more problems.
}



